Efficiently Hardening SGX Enclaves against Memory Access Pattern Attacks via Dynamic Program Partitioning

Intel SGX is known to be vulnerable to a class of practical attacks exploiting memory access pattern side-channels, notably page-fault attacks and cache timing attacks. A promising hardening scheme is to wrap applications in hardware transactions, enabled by Intel TSX, that return control to the software upon unexpected cache misses and interruptions so that the existing side-channel attacks exploiting these micro-architectural events can be detected and mitigated. However, existing hardening schemes scale only to small-data computation, with a typical working set smaller than one or few times (e.g., $8$ times) of a CPU data cache. This work tackles the data scalability and performance efficiency of security hardening schemes of Intel SGX enclaves against memory-access pattern side channels. The key insight is that the size of TSX transactions in the target computation is critical, both performance- and security-wise. Unlike the existing designs, this work dynamically partitions target computations to enlarge transactions while avoiding aborts, leading to lower performance overhead and improved side-channel security. We materialize the dynamic partitioning scheme and build a C++ library to monitor and model cache utilization at runtime. We further build a data analytical system using the library and implement various external oblivious algorithms. Performance evaluation shows that our work can effectively increase transaction size and reduce the execution time by up to two orders of magnitude compared with the state-of-the-art solutions.

==> main2.tex <==
%IEEE template


\ifdefined\TTTARGETaddon
  \begin{abstract}
  \input{text/0_abstract.tex}
  \end{abstract}
  \input{text/mainbody.tex}
\fi

\ifdefined\TTTARGETaddontwo
  \input{text/mainbody.tex}
\fi

\ifdefined\TTTARGETdone
  \input{text/abstract.tex}
  \input{text/introduction.tex}
  \input{text/background.tex}
  \input{text/mainbody.tex}
  \input{text/experiment.tex}
  \input{text/casestudy.tex}
  \input{text/relatedwork.tex} %related work should always be the last to write.
  \input{text/conclusion.tex}
\fi

\ifdefined\TTSTYLETARGETonecolumn
  \bibliographystyle{IEEEtran}
\fi
\ifdefined\TTSTYLETARGETieeetran
  \bibliographystyle{IEEEtran}
\fi
\ifdefined\TTSTYLETARGETsigalternate
  \bibliographystyle{abbrv}
\fi
\ifdefined\TTSTYLETARGETsig
  \bibliographystyle{abbrv}
\fi
\ifdefined\TTSTYLETARGETusenix
  \bibliographystyle{acm}
\fi

\ifdefined\TTSTYLETARGETreport
  \printbibliography
%note the list of bib is mentioned in sty/usepackage_config.tex
\else
  \bibliography{ads,lsm,yuzhetang,bkc,odb,cacheattacks,sc,crypto,sgx,diffpriv,txtbk,distrkvs,vc}
\fi

\ifdefined\TTUT
\ifdefined\TTSTYLETARGETsigalternate
  \appendix
\else
 \ifdefined\TTSTYLETARGETusenix
   \appendix
 \else
  \ifdefined\TTSTYLETARGETvldb
    \appendix
  \else
  \ifdefined\TTSTYLETARGETreport
    \appendix
  \else
    \ifdefined\TTSTYLETARGETllncs
      \appendix
    \else
      \appendices
    \fi
  \fi
 \fi
\fi
\fi

\input{text/appendix.tex}
\fi

\end{document}





==> sty/ieeetran/ieee-template/editable/README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sty/ieeetran/ieee-template/inputs/README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sty/ieeetran/titlepage.tex <==
\input{sty/title.tex}
\author{
\ifdefined\TTUT
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\fi
}

\maketitle
\IEEEpeerreviewmaketitle



==> sty/ieeetran/usepackage.tex <==
%using latex.XXX file to cusotmize style
%\usepackage{./sty/ieeetran/latex}



==> sty/llncs2e/titlepage.tex <==
\input{sty/title.tex}
\author{
Kai Li\hspace{0.25cm}
Yuzhe (Richard) Tang\hspace{0.25cm}
Beom Heyn (Ben) Kim$\ ^\dag{}$\hspace{0.25cm}
Jianliang Xu$\ ^\ddag{}$\hspace{0.25cm}\\
\ifdefined\TTUT
\fi
}

\institute{
    \fontsize{10}{10}\selectfont\itshape
    Syracuse University, New York, USA\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag{}$University of Toroto, Ontario, Canada\\
    \fontsize{10}{10}\selectfont\itshape
    $^\ddag{}$Hong Kong Baptist University, Kowloon Tong, Hong Kong 
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/titlepage.tex <==
\input{sty/title.tex}
\author{
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/usepackage.tex <==
\usepackage{etoolbox}
\makeatletter
\patchcmd{\chapter}{\if@openright\cleardoublepage\else\clearpage\fi}{}{}{}
\makeatother

\usepackage{titlesec}
{\filcenter\normalfont\Large\bfseries}
\titleformat{\chapter}
  {\normalfont\sffamily\LARGE\it}
  {\thechapter.}{10pt}{\LARGE}
\titlespacing*{\chapter}{0pt}{0pt}{0pt}
\titleformat{\section}
  {\normalfont\sffamily\Large\bfseries}
  {\thesection.}{0.3em}{}
\titleformat{\subsection}
  {\normalfont\sffamily\large\it}
  {\thesubsection.}{0.3em}{}





==> sty/sig-alternate/titlepage.tex <==
\input{sty/title.tex}
\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\numberofauthors{4} % if number of authors is bigger than number of \alighauthor used following, a ``addtional author'' section will be shown in the end of the paper.
%note: no empty line!
\author{
\alignauthor
Yuzhe Tang$^\dag$
%\titlenote{Author notes}
\\       \affaddr{Syracuse University}
\\       \affaddr{Syracuse, NY 13244}
\\       \email{$^\dag$ytang100@syr.edu}
\ifdefined\TTUT
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\and
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\fi
}
\date{30 July 1999}
\maketitle



==> sty/sig-alternate/titlepage_sharedAuthorAddr.tex <==
\begin{document}
%
\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
%
\linespread{0.9}

% --- Author Metadata here ---
\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\title{
Tang's Template of IEEEtran.cls for Conferences \titlenote{!Eye-catching title for high citation: make it short}
}

\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\numberofauthors{1}
\author{
\alignauthor Yuzhe Tang, Ting Wang and Ling Liu \\
  \affaddr{College of Computing, Georgia Institute of Technology} \\ 
  \affaddr{ Atlanta, GA 30332, USA} \\
  \email{yztang@gatech.edu, \{twang, lingliu\}@cc.gatech.edu}
}
\date{30 July 1999}
\maketitle



==> sty/title.tex <==
\begin{document}
% --- Author Metadata here ---
\title{\Huge Efficiently Hardening SGX Enclaves against Memory Access Pattern Attacks via Dynamic Program Partitioning}



==> sty/usenix/titlepage.tex <==
\input{sty/title.tex}

\ifdefined\TTUT
\author{
{\rm Your N.\ Here}\\
Your Institution
\and
{\rm Second Name}\\
Second Institution
% copy the following lines to add more authors
% \and
% {\rm Name}\\
%Name Institution
} % end author
\fi

\maketitle

% Use the following at camera-ready time to suppress page numbers.
% Comment it out when you first submit the paper for review.
\thispagestyle{empty}





==> sty/usenix/usepackage.tex <==
\usepackage{sty/usenix/usenix,epsfig,endnotes}


==> text/old/v1SYSTOR_2_approach.tex <==
\section{Related Work}

\subsection{Memory-Access Side-Channel Attacks}
\label{sec:background}

\noindent
{\bf Preliminary: TEE}: The architecture of SGX-alike TEE features a trusted world (a.k.a. enclave) and an untrusted world sharing a processor, the boundary between which is protected by some isolation mechanisms. The main memory usually resides in the untrusted world, where the content is protected by hardware encryption. 
In this TEE architecture, a memory reference has to access a series of micro-architectural ``buffers'', such as last-level cache (LLC), translation look-aside buffer (TLB), memory row buffer, etc., creating leakage side channels.

\noindent
{\bf Memory-access attacks}: A passive memory-access attacker monitors the access trace of an enclave execution and infers sensitive information. To monitor, the attacker {\it breaks} enclave execution and {\it observes} some micro-architectural side-channel. 
Existing memory-access attacks can be characterized by the spatial resolution of the leakage channel being observed and the temporal resolution of breaking the enclave control flow.
For instance, in the seminal work~\cite{DBLP:conf/sp/XuCP15}, 
a controlled page-fault attacker observes and breaks the enclave execution through page-fault interrupts, where the the trace' spatial granularity is page numbers and the temporal granularity is individual page accesses. 
More advanced attacks exploit other leakage channels (e.g., page-table access/dirty bits~\cite{DBLP:conf/uss/BulckWKPS17,DBLP:conf/ccs/WangCPZWBTG17}, shared last-level caches~\cite{DBLP:conf/usenix/HahnelCP17}) to improve spatial and temporal resolution. 
To make it harder to defend against, recent {\it stealthy} attacks break the enclave execution invisibly through hyper-threading that
eliminate interrupts~\cite{DBLP:conf/uss/GrussLSOHC17,DBLP:conf/ccs/WangCPZWBTG17}. 

\ignore{
\begin{figure}
\begin{center}
  \includegraphics[width=0.35\textwidth]{figures/sgxattacks-def.eps}
\caption{Taxonomy of memory-access attacks and defenses in SGX: {\small
Existing attacks shown in the diagram are code-named by the publication venue and year, including USS17 (USENIX Security)~\cite{DBLP:conf/uss/BulckWKPS17}, CCS17~\cite{DBLP:conf/ccs/WangCPZWBTG17}, SysTex17~\cite{DBLP:conf/sosp/BulckPS17}, ATC17~\cite{DBLP:conf/usenix/HahnelCP17}, OAKLAND15~\cite{DBLP:conf/sp/XuCP15}. Existing defenses shown in the diagram are code-named similarly and with their name, including T-SGX~\cite{shih2017t}, D\'ej\`a Vu~\cite{DBLP:conf/ccs/ChenZRZ17}, and Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}.
}}
\label{fig:sgxattacks}
\end{center}
\end{figure}
}

\subsection{Attack Mitigation by Isolation}

\noindent
{\bf Memory-access attack mitigation}:
A successful memory-access attack entails two conditions: 1) an observable channel of memory-access leakage, and 2) the capability of relating the leaked memory-access to sensitive information. A memory-access attack can be mitigated by breaking either condition: M1) Detecting that a leakage channel is being observed by {\it enclave fortification}, or M2) Eliminating the source of leakage by making it difficult to correlate the access trace with sensitive information, via {\it obliviousness}. 

{\color{black}
Existing mitigation techniques take different views regarding how side-channel attack works and takes action to close the leakage channel (i.e., isolation). SGX-LAPD~\cite{DBLP:conf/raid/FuBQL17} mitigates the page-fault attacks by enforcing that OS uses large pages. This property  of untrusted OS is verified by the enclave running a program to test the time of page fault. 

T-SGX~\cite{shih2017t} closes the page-fault channel by preventing interrupts in enclaves leveraging the TSX capability. Specifically, by wrapping computation into TSX transactions, any interrupt, including page faults that occur inside a transaction, will be captured by the software. T-SGX runs a policy that bounds the number of interrupts/page-faults to prevent page-fault attacks.

Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} and the work from Chen, et al~\cite{DBLP:conf/ccs/ChenLMZLCW18} close the cache side channels by detecting (individual) cache misses using TSX transactions.

Varys~\cite{DBLP:conf/usenix/OleksenkoTKSF18} reduces all existing side-channel attacks to two leakage channels, namely SGX's Asynchronous EXit (AEX) events and concurrent sharing of CPU cores. To close the first channel, it proposes to monitor the enclave AEX and terminates the enclave execution when the AEX frequency exceeds a threshold. It allocates sufficient hyperthreads to keep a CPU core occupied by a single application (so-called thread-core reservation) to close the second channel. Vary enforces the two conditions (AEX monitoring and thread-core reservation) in a trust-but-verify manner, that is, the OS is trusted to execute the program with the required property verified nevertheless by the enclave.
}

For the former, existing enclave-fortification work detects the attack on the events of page-fault~\cite{DBLP:conf/ccs/ShindeCNS16,shih2017t}, cache-miss~\cite{DBLP:conf/uss/GrussLSOHC17,DBLP:conf/woot/BrasserMDKCS17}, etc. 

For the latter, existing work on {\bf data-oblivious systems} is based on oblivious algorithms~\cite{DBLP:conf/nsdi/ZhengDBPGS17,DBLP:conf/ccs/OhrimenkoCFGKS15} or less-efficient oblivious RAM~\cite{DBLP:journals/iacr/SasyGF17,2017arXiv171000458E}.
Concretely, data obliviousness can eliminate the source of leakage in the presence of memory-access attacks on TEE. When building data-oblivious systems, a design choice is which oblivious-computing mechanisms to use: Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17} supports database queries by engineering word-oblivious algorithms (Column Sort~\cite{DBLP:journals/siamcomp/AzarV87}). Oblivious machine-learning~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16} combines word-oblivious algorithms and the trivial mechanism of converting random-access to a full-array scan. Scan-based transformation is similarly adopted in building ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}, an ORAM system in SGX. ObliVM~\cite{DBLP:conf/sp/LiuWNHS15} is a compiler that supports the engineering of both word-oblivious algorithms and ORAM~\cite{DBLP:conf/ccs/StefanovDSFRYD13,DBLP:journals/jacm/GoldreichO96}. Oblivious Map-Reduce~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15} and Prochlo~\cite{DBLP:conf/sosp/BittauEMMRLRKTS17} use external oblivious shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14} to protect distributed systems under traffic analysis, but insecure under micro-architectural memory-access attacks. 



\subsection{Attack Mitigation by Obliviousness}

\noindent
{\bf Data-oblivious algorithms}:  The conventional oblivious algorithms ensure oblivious data access at the ``word'' granularity. These {\it word-oblivious algorithms (A1)} are constructed based on primitives such as compare-exchanges and tend to be not very practical (e.g., AKS sorting~\cite{DBLP:conf/stoc/AjtaiKS83} and sub-optimal column sort~\cite{DBLP:journals/siamcomp/AzarV87}). In the external-memory model, {\bf external oblivious algorithms} improve the time/IO complexity by assuming a small amount of internal storage that is accessed in a leaky fashion. Due to a smaller constant and optimal complexity, this family of algorithms is of great practical interest. For instance,  Melbourne shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14} causes $O(\sqrt{N})$ IO with $O(N\log{N})$ time at the expense of $\sqrt{N}$ internal space and was recently used in constructing practical systems (e.g., MapReduce~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15}). Research to improve the algorithmic ``locality'' and to further reduce the internal-space complexity is underway~\cite{DBLP:journals/corr/abs-1709-07553}. The {\it oblivious RAM (A3)}~\cite{DBLP:conf/ccs/StefanovDSFRYD13,DBLP:journals/jacm/GoldreichO96} is an external data structure supporting oblivious external data access by translating virtual random-access to oblivious physical data access with poly-logarithmic blowup.

Comparing ORAM (A3) and word-oblivious algorithms (A1), the external oblivious algorithms (A2) cause lower overhead in complexity. Comparing generic ORAM, external oblivious algorithms are computation specific; existing algorithms support sort, compaction, and relational queries and other batched-oriented computations~\cite{DBLP:conf/icalp/OhrimenkoGTU14,DBLP:conf/ndss/WilliamsS08,DBLP:conf/spaa/Goodrich11,DBLP:conf/icdt/ArasuK14}.

\section{Research Formulation}

\subsection{System Model}
\label{sec:systemmodel}

\noindent
{\bf System model}: In this work, we consider the modern computing paradigm that a security-sensitive computation is outsourced and run on a third-party host. This paradigm becomes increasingly popular due to the advent of cloud computing, which has cost-effectiveness, availability, etc. Concretely, the data owner possessing security-sensitive personal data uploads the data and program to a third-part host in the cloud where the program is executed over the data to evaluate the computation on the owner's behalf.

The host in our system has an SGX-alike trusted execution environment or enclave. The enclave is trusted by the data owner, including the processor at the hardware layer and the owner-provided program at the software layer. Hardware and software outside this perimeter of the enclave is untrusted by the data owner. 

\label{sec:computation}
{\bf The target computation} of this work is what we call external-oblivious computation. The working set of this computation consists of a large volume of data accessed in a non-leaky fashion (named non-leaky data) and a small volume of data accessed in a leaky fashion (named access-leaky data). The small volume of access-leaky data is defined to be cache resident. 

In practice, we deem there are a large number of real-world applications that meet the external-oblivious computations, especially in data-analytical applications. For instance, streaming applications feature a big-data stream that is accessed in a non-oblivious fashion while keeping a small state that is accessed randomly (or in a leaky fashion). In other data-analytical computations,\footnote{Data analytical algorithms usually have super-linear time complexity and need to access data in multiple iterations.} a common paradigm is to iterate through the dataset multiple times, each of which runs a stateful computation with a data pass through the dataset. Even for computations that are not natively external-oblivious, such as sorting (quick sort or merge sort are not oblivious), there are external oblivious algorithms, such as Melbourne shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14}, oblivious merge sorts~\cite{DBLP:conf/ndss/WilliamsS08}. We conduct a study of a series of related cases and support sample external-oblivious computations in \S~\ref{sec:cases}. 

Out of the scope is the computation that randomly accesses a large external dataset, such as database search (with index); these computations can be supported by existing work such as ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17} that engineers an ORAM in external storage.

\subsection{Threat Model}
\label{sec:threat}
This work considers memory-access pattern attacks in the emerging hardware enclaves. A program runs inside an enclave of a trusted processor and encrypted memory in the target system, and the adversary monitors certain micro-architectural side-channel during the enclave execution. Based on the observed access trace, she then infers other sensitive information.
The exploited leakage channels include page-fault~\cite{DBLP:conf/sp/XuCP15}, page-table access/dirty bits~\cite{DBLP:conf/uss/0001SGKKP17,DBLP:conf/uss/BulckWKPS17}, cache-timing~\cite{DBLP:conf/ccs/WangCPZWBTG17,DBLP:conf/usenix/HahnelCP17}. 
Access-driven attacks against data-intensive computations can lead to significant information disclosure~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15,DBLP:conf/nsdi/ZhengDBPGS17,DBLP:journals/corr/BaterEEGKD16}.
For clarity, the non-goals of this work include other side-channel attacks (e.g., timing attacks, power analysis), denial-of-service attacks, rollback attacks, etc.

\subsection{Security Goal}
\label{sec:cmo}

Intuitively, the cache-miss obliviousness or CMO requires that the trace of cache-misses (as exposed in bus-tapping attacks) in a program execution should be independent with any execution data (both input and intermediate data). Consider executing a program $P$ with data $I$. The execution produces trace $T$ consisting of last-level cache misses. CMO requires that given two data values, $I_0$ and $I_1$, a CMO execution produces two identical traces, that is, $T_P(I_0)=T_P(I_1)$. 
This definition assumes that the computation induced by $P$ is deterministic. And the definition of obliviousness is ``perfect'' as it requires the two traces of different data are exactly the same.
We skip the more formal and generic definition of cache-miss obliviousness (e.g., based on indistinguishability formation~\cite{DBLP:books/crc/KatzLindell2007}). 

\subsection{Research Problem}

The focus of this work is the support of efficient data-intensive computations (in \S~\ref{sec:computation}) with cache-miss obliviousness (in \S~\ref{sec:cmo}) on the TEE platforms (in \S~\ref{sec:systemmodel}). Particularly, the cache-miss obliviousness ensures the memory-access security under cache-timing attacks while retaining external-oblivious algorithms' efficiency.

This goal presents an open research problem: Existing research on cache-timing attack detection (e.g., by HTM) is limited in data scalability as the working set must be cache-resident. Existing research on data-obliviousness engineering largely focuses on word-oblivious algorithms (e.g., Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17}, ObliviousML~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16}). The limited work considering the more efficient external-oblivious algorithms (e.g., ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}, ObliviousMR~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15}, Prochlo~\cite{DBLP:conf/sosp/BittauEMMRLRKTS17}) has either sub-par security or sub-optimal performance efficiency.

We survey existing research from the angles of strong cache-attack security, data scalability, and algorithmic complexity. The research distinction of our work is presented in Table~\ref{tab:distinct}.

\begin{table*}[!htbp] 
\caption{Research distinction}
\label{tab:distinct}\centering{
\small
\begin{tabularx}{0.9\textwidth}{|c|c|X|X|X|}
  \hline
 & Method
 & Cache access-pattern security 
 & Data scalability 
 & Algorithmic complexity \\ \hline
  T-SGX~\cite{shih2017t}, Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}
  & Attack detection by HTM & + & - & + \\ \hline
  Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17}, ObliviousML~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16}
  & Word-oblivious algo. & + & + & - \\ \hline
  ObliviousMR~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15},Prochlo~\cite{DBLP:conf/sosp/BittauEMMRLRKTS17}
  & External oblivious algo. & - & + & + \\ \hline
  ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}
  & External ORAM & + & + & - \\ \hline
  This work
  & External oblivious algo./HTM & + & + & + \\ \hline
\end{tabularx}
}
\end{table*}

\ignore{
\subsection{Proposed Method}
\label{sec:approach}
Our method for engineering external obliviousness is that given the target computation expressed by an external-oblivious algorithm, we place and only place the part of the program accessing internal memory in external-oblivious algorithms to the HTM transactions. By this means, the cache-misses which only occur between transactions are oblivious, while cache-hits and other internal accesses can be made secure by HTM protection.

The motivation to combine HTM and external oblivious algorithms can be better illustrated by an example: Consider implementing a sort on Intel SGX with cache-attack security. The first baseline (BL1) entails implementing the word-oblivious sorting network at the expense of a logarithmic multiplicative factor (i.e., $O(N\log^2{N})$). The second baseline is to use HTM to protect the leaky accesses in a classic sorting algorithm of $O(N\log{N})$ complexity, such as quicksort or merge sort. This approach limits the data size by CPU cache size. In a big-data setting (with large $N$), neither approach is feasible as the former is inefficient and the latter is unscalable. By contrast, our proposed method combining HTM and external oblivious algorithms could lead to an optimal $O(N\log{N})$ sorting algorithm (based on the scramble-then-shuffle paradigm~\cite{DBLP:journals/popets/DangDCO17}) implemented with cache-attack security.

Note that our approach shares some general ideas with Cloak and T-SGX in the sense that it leverages Intel TSX to detect memory-access attacks. However, Cloak does not automatically partition the computation and is limited to the small-data case. T-SGX is a static program-partition scheme, which limits its applicability in handling loops and thus big-data computations. Our work uniquely addresses the problem of dynamically partitioning the programs to support big-data computations with access-pattern security.
}

\section{System Overview}
Our goal is to build a data-intensive runtime system with access-pattern security on hardware enclaves. Concretely, given an external oblivious algorithm, we provide an API (S1) for developers to annotate the leaky section of the program. Given the annotated program, we provide an execution engine (S2) that runs the program on the architecture of two execution environments: the one with access-pattern protection (e.g., prohibiting cache-misses) and the other without. We call the former by fortified enclave and the latter by unprotected enclave. Briefly, the execution engine partitions the runtime instance dynamically in a way that assures no cache-miss yet can scale to relatively large data.
Figure~\ref{fig:overview} illustrates the overview of our system. In the following, we present the detailed design and implementation of our system in each component, S1 in \S~\ref{sec:api} and S2 in \S~\ref{sec:dynpart}.

\begin{figure} 
\centering
\includegraphics[width=0.26\textwidth]{figures/system-overview.eps}
\caption{System overview: A target computation is annotated by our programming API that specifies data-access pattern. Our runtime system first partitions the program dynamically to units (i.e., dynamic partitioning), and then runs each unit in an TSX transaction (i.e., tx-execution engine).}
\label{fig:overview}
\end{figure}

\noindent
{\bf Preliminary: External-oblivious algorithms}
\label{sec:prel:externalobl}
External oblivious algorithms are a class of oblivious mechanisms that has advantageous time complexity at the expense of assuming a trusted internal memory. External oblivious algorithms are proposed for a wide variety of computations, including shuffle (Melbourne shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14}), sort (oblivious merge sort~\cite{DBLP:conf/ndss/WilliamsS08}), most aggregation computations, etc. Comparing word-oblivious algorithms (e.g., sorting networks causing a multiplicative factor of $O(\log{N})$), an external oblivious algorithm has better time complexity (e.g., Melbourne shuffle based sorting~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15,DBLP:journals/popets/DangDCO17} with the O(1) multiplicative factor). Comparing ORAM (with a multiplicative factor of $O(\log^2{N})$), an external oblivious algorithm is specific to target computation and is more efficient.
While external oblivious algorithms achieve better complexity, they may present limitations on data scalability. Concretely, most existing external oblivious algorithms are designed for a client-server setting and assume a large internal memory at the client side. For instance, a Melbourne shuffle assumes an internal memory of $O(\sqrt{N})$. The large internal memory may be suited for a client machine (in the big-data setting), but presents challenges when treating cache as internal memory, whose size is very limited; for instance, a L1 cache is 32 KB and L3 cache is 8 MB in an Intel SGX CPU. Very recently, space-efficient external oblivious algorithms are proposed, for instance, stash shuffle with small $O(\log{N})$ internal space.

\noindent
\label{sec:api}
{\bf API}: Our system provides a programming interface for C++ developers to annotate the leaky section of the program and define the type of data referenced inside the leaky section. Specifically, 1) we provide two library functions, \texttt{begin\_leaky()} and \texttt{end\_leaky()}, for developers to declare the begin and end of a program snippet where leaky memory access occurs. 2) In addition, all the memory data accessed inside a leaky section needs to be defined with our data type. We provide four data-container types as defined below. The explicit data type allows our execution engine to be know ahead of time the possible data-access pattern and take action in partitioning more precisely.

The data-container types are classified based on whether the access is leaky and whether the data is read-only. The four data types are \texttt{NobRO}, \texttt{ObRO}, \texttt{NobRW}, \texttt{ObRW}, where \texttt{ObRW} stands for oblivious read-write data container and NobRO is non-oblivious read-only data container. The API of the data classes are provided in Figure~\ref{lst:samplecode}. We also provide an example code that declares the merge passes in a merge sort algorithm to be leaky sections.

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
class ObRO {
  int32_t read_next(); 
  void reset();
}
class ObRW {
  void write_next(int32_t data); 
  void reset();
}
class NobRW {
  int32_t read_at(int32_t addr);
  void write_at(int32_t addr, int32_t data); 
}
class NobRO {
  int32_t nob_read_at(int32_t addr); 
}
\end{lstlisting}
\end{minipage}
\\
\vspace{-0.35in}
\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
void MergeSort(int[] array, int start, int end){ 
  if (start == end - 1) return;
  MergeSort(array, start, (end + start)/2); 
  MergeSort(array, (end + start)/2, end);
  Merge(array, 0, (end + start)/2, (end + start)/2, end);
}
void Merge(int[] array, int start1, int end1, int start2, int end2){
  *NobRW* parray = new *NobRW*(array);
  *begin_leaky();*
  originalMerge(parray, start1, end1, start2, end2); 
  *end_leaky();*
}
\end{lstlisting}
\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Implementing merge sort based on the CMO API: in-transaction data types and leaky section}
\label{lst:samplecode}
\end{figure}

\section{Dynamic Program Partitioning}
\label{sec:dynpart}

\subsection{Motivation}

Existing side-channel defenses leverage the hardware transaction features to detect any unintended cache misses. Notably, Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} detects cache attacks using Intel TSX. Briefly, it executes the computation in HTM transactions, such that the intra-transaction memory accesses are resolved by cache hits and thus are concealed from the adversary. Note that the inter-transaction memory accesses are disclosed. The security of these Cloak alike schemes requires that access-leaky memory region must reside in data cache; this security requirement significantly limits the data scale. In addition, Cloak's programming interface is rather low-level and requires the programmer to manually specify the scope of individual HTM transactions, which further limit its applicability in big-data computations.

To systematically improve the data scalability, we study two technical problems: (O1) dynamic program partitioning and (O2) enlarging transaction. First, given a target computation, we dynamically partition the program to smaller execution units, each run in an individual transaction. Comparing existing work, such as Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} and T-SGX~\cite{shih2017t}, our unique perspective about program partitioning is to take into account various runtime information (see \S~\ref{sec:approach} for detailed comparison). 

Second, for each execution unit, we enlarge the transaction as much as possible. Here, the larger a transaction is, the performance efficiency it can be, as the transaction setup cost (e.g., running \texttt{xbegin}/\texttt{xend} instructions) can be amortized among more instructions. Note that the size of any TSX transaction has a theoretic limit in that its working set cannot exceed a CPU data cache. Our goal is to reach this theoretic bound in transaction size. 

\subsection{Dynamic Partitioning Problem}

As revealed in our API design in \S~\ref{sec:api}, a starting point of our approach is to expose to the runtime system some high-level semantic information. This information includes different types of data accesses; concretely, the data-container types in our API lets the runtime be aware of four data-access classes: 1) non-oblivious reads (or access-leaky reads as in \texttt{NobRO}), 2) non-oblivious writes (or access-leaky writes as in \texttt{NobRW}), 3) oblivious reads (as in \texttt{ObRO}) and 4) oblivious writes (as in \texttt{ObRW}). 

With awareness of data access type, we can specify the constraints of program partitioning problem. In general, there are two constraints, the constraint imposed by the TSX hardware (C1) and that imposed by the security requirement (C2). 
Figure~\ref{fig:constraints} illustrates the two constraints in the presence of four types of data accesses. 
For C1, it requires that a transaction's write-set should not cause L1 cache replacement, and a transaction's read-set should not cause LLC cache replacement. For C2, the access-leaky memory region must reside in data cache without being split.  Here, an access-leaky memory region is defined by memory data accessed in a data-dependent way; for instance, \texttt{NobRO} and \texttt{NobRW} instances are access-leaky regions.\footnote{We may use terms \texttt{NobXX} to represent access-leaky regions} The constraint of C2 is due to the strong security concern. Because the HTM based protection only conceals the intra-transaction memory access pattern, and the inter-transaction memory access pattern is disclosed. Placing the leaky memory accesses across multiple transactions would inevitably disclose the data secrets. 

\begin{figure} 
\centering
\includegraphics[width=0.35\textwidth]{figures/constraints.eps}
\caption{Transactional data constraints imposed by hardware (C1) and security (C2) requirements. The data is classified to four types based on read/write and leaky/non-leaky.} 
\label{fig:constraints} 
\end{figure}

Because of the constraints (particularly C2), we focus on \emph{partitioning the non-leaky part of the program}. That is, we consider the problem of partitioning the program into smaller units, each unit accessing a partition of non-leaky data (\texttt{ObXX}) but accessing leaky data in their entirety. Note that the leaky data is not partitioned and has to be loaded in total to the data cache. This design choice implies that we only support computation with small cache-bound leaky data (\texttt{NobXX}).\footnote{Note that the assumption presents a fundamental limitation of our approach in supporting computation of large access-leaky data.}, which is consistent with our target computations (as described in \S~\ref{sec:computation}).  

Our goal is two-fold: (O1) Support computations of (non-leaky) data as large as possible by dynamically partitioning the computations, 
and (O2) Run these computations using transactions of as large size as possible.

The high-level approach is illustrated in Figure~\ref{fig:shadow}. As in the figure, consider a computation whose application memory consists of (cache-bound) access-leaky data (i.e., A1 and A2) and large non-leaky data (i.e., A3 and A4). We split the non-leaky data into a series of smaller data partitions (i.e., \{P3\} and \{P4\}), each of which is small enough to fit in a CPU data cache. 
To support large transactions (O2), we enable \emph{L1 cache replacement on read-only data}. That is, the footprint of A1 and P3 in L1 cache can be reduced to just one set, as will be explained next.

\fbox{\parbox{0.90\linewidth}{
Formally, our work can be formulated as an optimization problem: Given a program $G$ on data $\{A1,A2,A3,A4\}$, it partitions $G$ to a series of $\{g\}$ with each program partition $g$ operate on data $A1,A2,P3,P4$ such that it maximizes $\min{P3,P4}$ and it is subject to the following constraints:

\begin{eqnarray}
  \nonumber
\cup\{P3\} & = & A3\\
  \nonumber
\cup\{P4\} & = & A4\\
  \nonumber
A1 + P3 + A2 + P4 & < & LLC\\
  \nonumber
A1/L + P3/L + A2 + P4 & < & L1
\end{eqnarray}

Here, $L$ is the maximal number of LLC cache lines that can be mapped to one L1 cache set.
}}


\subsection{Supporting Large Transactions by Shadow Memory}
\label{sec:shadowmem}

As will be described next, read-only data (A1 and P3) in a transaction can reuse L1 data cache without aborting the transaction. 

%cache full utilization is essential.\footnote{For instance, a poorly utilized cache may abort a transaction when just one set (out of say 64 cache sets) is full. A well-utilized cache may abort a transaction when the entire cache is full, which results in a much larger transaction.} 

Efficient use of the cache is of particular importance to ensuring large transactions. The transaction will not abort when the cache is underutilized; for instance, the transaction may end when only one cache set (out of 64) becomes full while the other sets are empty.

We propose a technique called shadow memory that arranges the in- transaction memory layout such that memory data is mapped to the CPU cache hierarchy without unnecessary conflict. Briefly, we enforce the rules that different types of data (A1, ...A4) should not overlap in data caches. Specifically, consider a cache hierarchy with a 8-way 32KB L1 cache and 16-way 8MB L2 cache. We allocate 60 L1C sets to be A2 (\texttt{NobRW}), 2 L1C sets to be P4, 1 L1C set to be P3 and L1C set to be A1. Note that A1 and P3 can reuse the L1 cache and their sizes are bounded by LLC. Figure~\ref{fig:shadow} illustrates an example of shadow memory.

\begin{figure} 
  \centering
  \includegraphics[width=0.475\textwidth]{figures/shadow_memory_cache.eps} 
  \caption{Splitting data to transaction-wise partitions and mapping data in memory/cache hierarchy: Shadow-memory is an indirection layer that arranges data in cache based on access pattern. From LL (Last-Level) cache to L1 (Level-one) cache, read-only data replacement is enabled.} 
\label{fig:shadow} 
\end{figure}

\subsection{Implementing Dynamic Partitioning}

When realizing the dynamic partitioning, we encountered two design problems: 1) How and when to insert the \texttt{xbegin} and \texttt{xend} instructions to properly declare transaction boundaries such that the transactions can successfully finish their execution (i.e., without abort) yet are not prematurely ended? 2) How to realize the shadow memory in its full life cycle? 3) How to decide the condition that the computation cannot be executed using transactions at an early time (e.g., when the A1 is larger than LLC).

We build a library that realizes the partitioning life cycle. Recall that our API supports declaring the leak section's scope and wrapping each in-transaction memory access by custom data types. Upon leaky section declaration, we realize the allocation of shadow memory. Upon the in-transaction memory access, we hook the transaction partitioning schemes. The overall mechanism is illustrated in Figure~\ref{fig:libimpl}, and pseudo-code is presented in Listing~\ref{lst:samplecode:hook}.

\begin{figure} 
  \centering
  \includegraphics[width=0.4\textwidth]{figures/lib_impl.eps}
\caption{Library implementation: Each box represents a function in our library. White boxes run outside TSX transactions and blue boxes run inside TSX transactions.} 
\label{fig:libimpl} 
\end{figure}

Concretely, for shadow memory allocation, we allocate the shadow memory according to the layout described in \S~\ref{sec:shadowmem}. Note that the shadow-memory size is fixed (as the total size of a cache is fixed). We perform checks on whether the data size, specifically the size of access-leaky memory data, is small enough to fit into the data cache. In other words, we enforce the constraint C1 that A1 does not exceed L1 and A2 does not exceed LLC.

For transaction partitioning, we implement two components: 1) monitoring cache usage, and 2) realizing transaction partitioning. For 1), we simply monitor the condition that if each non-leaky data overflows, that is, the iterator call to \texttt{ObXX.next()}\footnote{\texttt{ObXX} refers to non-leaky data type, either \texttt{ObRO} or \texttt{ObRW}.} reaches its capability. Note that we enforce a joint capability limit, that is, the total size of \texttt{ObXX} objects is bounded instead of individual \texttt{ObXX}.

For 2), we insert the TSX instructions \texttt{xend} and \texttt{xbegin}. Between them, we make data copy between shadow memory and application memory of the non-leaky data. Because the computation is partitioned based on non-leaky data, different transactions in the same leaky-section computation will use different non-leaky data, thus making it necessary to reload non-leaky data across transactions. Also, we perform \emph{double preloading} across the transactional boundary.

\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  caption={Library implementation: hooking dynamic-partitioning trigger in non-leaky data scans.},                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  label={lst:samplecode:hook},
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
begin_leaky(){
 shadow_memory_alloc();
}
ObXX::next(){
  //dynamically partition computations in next();
  //1. monitoring the overflow
  if(shadow_mem.ob.size + 1 < shadow_mem.ob.capability()) return;
  //2. start to execute the partitioning
  xend();
  //reload non-leaky data (ob) in shadow memory from application memory
  shadow_mem.reload_ob();
  double_preload();
  xbegin();
}
\end{lstlisting}

\section{Case Studies}
\label{sec:cases}

Our system supports external-oblivious computing. In our perspective, some computations are natively external-oblivious, such as binary search, iterative machine learning, etc.. There are some computations whose classic algorithms are not oblivious, but there exist external-oblivious algorithms. For instance, for sorting, the most common algorithms, such as quicksort, are not oblivious. There are external-oblivious sorting algorithms, such as oblivious merge sort and Melbourne shuffle-based sort, that have the same $O(N\log{N})$ complexity with quicksort. 

In this section, we present our experience building various external-oblivious computations using our library. 

\noindent{\bf K-means}:
A K-means computation takes as input a data array and randomly initialized K centroids. It produces the output of K centroids in K clusters that are the most representative of the data array. Here, each element in the data array represents a data point, and there are pair-wise distances defined between them. The key-means computation runs iteratively, where each iteration consists of two data passes, one (KM1) is a nested loop that (re)-assigns every array element to the closest centroid, and the other (KM2) is an array scan that randomly accesses the centroid array to update the centroid position. 

K-means is an external oblivious computation in the sense that it keeps the centroid as internal memory accessed in a leaky way and the data array as an external memory, which is accessed obliviously. 

To implement K-means using our library, we declare the data pass (KM2) to be the leaky section where the internal memory is accessed. In the leaky section, the centroid array is defined as a NobRW, data array as an \texttt{ObRO}, the data-centroid mapping as an \texttt{ObRW}. 
%The related sample code is in Listing~\ref{XXX}.

\noindent{\bf Melbourne shuffle}:
A Melbourne shuffle is a randomized algorithm for data shuffling. A data-shuffle operation takes as input two arrays of equal length, one storing data and the other storing a permutation. It produces the output of permuted data array. For instance, $\texttt{mshuffle}({x,y,z},{1,0,2})={y,x,z}$. Internally, Melbourne shuffle is a randomized algorithm that bucketizes each of the two arrays to $\sqrt{N}$ buckets, each of $\sqrt{N}$ size. A Melbourne shuffle runs in two rounds, each round using $\log{N}\sqrt{N}$ internal memory accessed in a leaky fashion. The original input arrays are in external memory.

To implement Melbourne shuffle using our library, we declare both rounds to be leaky sections. In particular, for scalability, we declare the first round, which is to ``distribute data bucket based on permutation bucket'', to be two leaky sections. Briefly, the first leaky section in the distribution round produces the unordered, linked list as output, without dummy elements. The second leaky section adds dummy elements. In this way, we can improve the data scalability significantly and reduce the access-leaky internal memory from $O(\log{N}\sqrt{N})$ to $O(\sqrt{N})$.   

\noindent{\bf Oblivious merge sort}:
In oblivious merge sort, the operation of merging two sorted lists is made oblivious by a randomized algorithm~\cite{DBLP:conf/ndss/WilliamsS08}. Given two sorted lists, an oblivious merge keeps a $O(\sqrt{N})$ internal-memory buffer and finishes the merge computation with the same $O(N)$ complexity. It is a randomized algorithm and the probability of internal buffer overflowing is made negligible.  

We implement oblivious merge sort by declaring the merge operation to be leaky section and the internal buffer to be a \texttt{NobRW} and the two merging arrays to be two \texttt{ObRO}.

\noindent{\bf 
Streaming binary search}:
Consider a query on a sorted data array. A binary search locates the matching element in the array to the query. Given a stream of queries, the binary search can be treated as an external-oblivious process in the sense that the internal memory maintains the data array, and external memory maintains the query stream.

To implement the streaming binary search using our library, we declare the binary search to be the leaky section, the data array to be a \texttt{NobRO}, the query stream (array) to be an \texttt{ObRO}. 

\section{Performance Evaluation}

In this section, we evaluate our system in terms of data scalability and performance. We first conduct a micro-benchmark study on the transaction success rate. We then conduct a macro-benchmark study that extensively evaluates the system performance under different data scales. 

\subsection{Micro-Benchmark}

\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{figures/exp-Executiontime-Datasize.eps}
\caption{Performance under varying transaction sizes}
\label{exp:txsize}
\end{figure}

In this micro-benchmark study, we evaluate the performance with varying transaction sizes. Speculatively, a small transaction would cause high-performance overhead. 

For this experiment, we consider a simple computation of a loop writing to a data array. Each array element has a cache line size, such that each element access leads to a cache miss. We control the transaction size by the number of elements accessed. 

We run the program on an Intel SGX machine with the following specs:  Intel(R) Core(TM) i5-7500 CPU @ 3.40GHz 64 bits, with 32 KB L1 cache size (8-way 64 sets) and 8 GB RAM. In the experiment, we vary the size of the transaction and the data size (i.e., the array length). We conduct the program run 1000 times and measure the average execution time and its standard deviation.

The performance result is presented in Figure~\ref{exp:txsize}. With increasing transaction sizes, the execution time generally decreases. Specifically, when transaction size increases from 8 to 64, the execution time decreases by 2 - 5 times. When the transaction grows beyond 1024, the execution time becomes very unstable. When the transaction size is 2048 cache lines, the execution is limited for small data, such as below 256 cache lines.

The reason for performance improvement with increasing transaction size is that the cost of transaction setup (e.g., running \texttt{xbegin} and \texttt{xend}) is amortized over more instructions with larger transactions. When a transaction grows over a threshold, the return (of performance increase) diminishes. And if the transaction grows too large (e.g., larger than cache size), the transaction abort rate will increase due to cache replacement in transactions, which leads to unstable execution and large execution time.

\begin{figure*} 
\centering
\subfloat[Binary search: Number of queries]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofqueries.eps}
  \label{exp:bs:query}
}
\subfloat[Binary search: Number of records]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-binarysearch.eps}
  \label{exp:bs:data}
}
\subfloat[K Means: Number of records]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-kmeans.eps}
  \label{exp:kmeans:data}
}
\subfloat[K Means: Number of centroids (K)]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Valueofk.eps}
  \label{exp:kmeans:k}
}
\caption{Comparing CMO with scan: Binary searches and k-means}
\label{exp:vsscan}
\end{figure*}

\begin{figure}
\subfloat[Melbourne shuffle]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-melbourne.eps}
  \label{exp:melbourne:data}
}
\subfloat[Oblivious merge sort]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-mergesort.eps}
  \label{exp:oms:data}
}
\caption{Comparing CMO with scan: External-oblivious sorts}
\label{exp:vsscan2}
\end{figure}

\begin{figure} 
\centering
\includegraphics[width=0.5\textwidth]{figures/exp-Executiontime-Numberofrecords-sorting.eps}
\caption{Comparing CMO with word-obliviousness and Cloak: the case of sorting}
\label{exp:sorting}
\end{figure}


\subsection{Macro Benchmark}

\noindent{\bf Comparison with scan baseline}: 
This set of experiments evaluates the performance of CMO, in comparison to scan-based baselines.  The scan-based baseline translates each leaky random access (on \texttt{NobXX}) to a full array scan. Note that while ORAM~\cite{DBLP:conf/ccs/StefanovDSFRYD13,DBLP:journals/jacm/GoldreichO96} presents a generic solution with better (asymptotic) efficiency, the scan-based data-obliviousness approach is the state-of-the-art; it is implemented more widely for in-memory data processing due to its simplicity, such as in oblivious machine learning~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16} and ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}\footnote{ZeroTrace uses ORAM for disk data access and scan for its internal-memory data access.}. In addition, at a medium data scale, the better asymptotic efficiency of ORAM may not translate to better concrete performance. We implement the scan baseline in our library by converting each access to \texttt{NobXX} to a full-array scan.

We consider the various computations in our case study. In each experiment, we measure the performance by execution time. Specifically, the execution time only includes the time spent on executing the computation and excludes the time spent on data loading and system initialization. We use numeric datasets and generate them randomly. 

We did all the experiments on a laptop with an Intel 8-core i7-6820HK CPU of 2.70GHz, 32KB L1 and 8MB LL cache, 32 GB RAM, and 1 TB Disk. This is one of the Skylake CPUs equipped with both SGX and TSX features. 

We vary the data size in each computation and report the results in Figures~\ref{exp:vsscan} and ~\ref{exp:vsscan2}. 
Figure~\ref{exp:melbourne:data} and ~\ref{exp:oms:data} evaluate the execution time of Melbourne shuffle and oblivious merge sort. Comparing the baseline of scan approach, the Melbourne shuffle by CMO achieves a speedup of more than 100X at the largest data scale of 1 million records. For oblivious merge sort, the speedup is much less significant, about 10% speedup of the baseline. 
%The reduced speedup is related to the fact that XXX. 

Figures~\ref{exp:bs:data} and~\ref{exp:bs:query} present the performance result of streaming binary search with varying data size and the number of queries. With varying data size, the CMO outperforms the scan baseline by a speedup ranging from 100X to 1000X. With varying query numbers, CMO first keeps the execution time constant until the cache cannot accommodate all the queries. CMO's execution time then linearly scales with the query number. With a large query number, CMO outperforms the scan baseline by 1000X times. Similarly, the performance result of K-means in Figures~\ref{exp:kmeans:data} and~\ref{exp:kmeans:k} also show multi-magnitude speedup of CMO.

\noindent{\bf Comparison with other algorithms}:
In this set of experiments, we evaluate the importance of dynamic partitioning by measuring the performance of CMO against two baselines without partitioning: 1) pure data-obviousness approach and 2) TSX based attack-detection (as in Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}). We allow one to choose the best and most-efficient algorithm in each baseline. For TSX attack detection, we consider quick sort. For data-oblivious computing, we consider bubble sort. For CMO, we consider three sorting algorithms, Melbourne shuffle with quick sort (following the scramble-then-compute paradigm~\cite{DBLP:journals/popets/DangDCO17}), oblivious merge sort, and cache shuffle with quicksort.

The performance result is in Figure~\ref{exp:sorting}. It can be seen that the TSX attack detection is limited in data scalability. The baseline of bubble sort causes high  overhead, especially as data size grows. The CMO paradigm, with different algorithms, achieves much better performance than the baselines with up to two orders of magnitudes speedup.

\section{Conclusion}
This work enables cache-miss oblivious data analytics with Intel SGX. It considers expressing target data analytics by external oblivious algorithms and protect their stash's memory access pattern by dynamically partitioning the code and wrapping them in TSX transactions. 
We develop a C++ library that monitors  memory accesses and builds a cache model to predict cache misses. 
On the library, we implement various various external oblivious algorithms.
The evaluation shows effectively increased transaction size and reduced execution time by orders of magnitude in comparison with the state-of-the-art systems.


==> text/old/v1_intro.tex <==
\section{Introduction}
In today's trusted execution environments (TEE), notably Intel SGX, memory content is encrypted with the intent to protect data confidentiality against a priviledged adversary (e.g., with control of the operating system).
However, recent practical attacks on SGX have demonstrated the feasibility of extracting the plaintext of memory content by observing the memory access pattern disclosed through various micro-architectural side channels (e.g., page fault, cache timing, et al~\cite{DBLP:conf/sp/XuCP15,DBLP:conf/uss/BulckWKPS17,DBLP:conf/uss/0001SGKKP17,DBLP:conf/ccs/WangCPZWBTG17}). Protecting memory access pattern against such side-channels becomes the last defense and is critical to the overall TEE security.

Software-only defense is advantageous for practitioners to deploy on off-the-shelf TEEs. A promising defense design is (ab)using Intel hardware transactional memory (TSX), a feature that many Intel SGX CPUs support, for side-channel defenses. Briefly, TSX guarantees that if a cache miss occurs when program executes inside a hardware transaction, the transaction will be aborted with control returned to the software. Thus, the successful execution of a TSX transaction implies no cache misses during the execution, thus no leakage of memory access pattern.
%
Following this design, existing systems such as Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} and D\'ej\`a Vu~\cite{DBLP:conf/ccs/ChenZRZ17} target the support of cryptographic algorithms and wrap them in transactions using manual annotation and domain knowledge (e.g., identifying a procedure of small working set, such as symmetric encryption, and executing it in one transaction).
%
Beyond cryptographic operations, the primary applications of TEE are those that conduct generic computation on top of sensitive data. In this case, automatic program partitioning is required. T-SGX~\cite{shih2017t} employs a static program partitioning scheme, which works as an LLVM extension and inserts TSX instructions to target programs to declare transactional boundaries.
To avoid (deterministic) transaction aborts, T-SGX limits the number of memory instructions per partition. At the compilation time, T-SGX has to consider the worst case of runtime and conservatively sets the maximal number, such as 8 load/store instructions per partition for an 8-way cache. If more than $8$ memory instructions are packed to a partition, the worst-case scenario can occur: running the partition always causes a cache miss and thus aborts the transaction.
As a result, transactions generated from static partitioning schemes are rather small, which further leads to fine-grained information leakage and degraded confidentiality protection. 
%See XXX for details.

This work tackles the security hardening of TSX-based side-channel protection towards enabling secure data analytics in Intel SGX enclaves.
One particular goal is to enlarge the transaction to fully utilize the CPU cache. 
Ideally, a transaction can be enlarged to include as many instruction as the next instruction to include does not cause cache miss (which further triggers transaction aborts). 
The proposed approach is to dynamically insert transaction boundary instructions instead of statically as in the existing works. In dynamic program partitioning, the motivating observation is that runtime information, such as current cache utilization, can be leveraged to predict the next cache miss, more precisely, to result in larger TSX transactions.
The design comparison of our dynamic program partitioning and existing methods is presented in Table~\ref{tab:distinction}.

\begin{table}[!htbp] %force in current page, disable float.
\caption{Design comparison}
\label{tab:distinction}\centering{\footnotesize
\begin{tabularx}{0.425\textwidth}{ |c|X|X|X| }
  \hline
Systems & Partitioning method & Generic computation & Side-channel defense 
  \\ \hline
Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}
& 
\multirow{2}{*}{Manual} 
&
\multirow{2}{*}{\xmark} 
& 
\multirow{2}{*}{\xmark} %(Cache-timing attacks only)
  \\ \cline{1-1}
D\'ej\`a Vu~\cite{DBLP:conf/ccs/ChenZRZ17} 
& & & \\ \hline
T-SGX~\cite{shih2017t} & Static & \xmark  & \xmark %(Page-fault attacks only)
  \\ \hline
This work & Dynamic & \cmark & \cmark
  \\ \hline
\end{tabularx}
}
\end{table}

We develop a C++ library to materialize dynamic program partitioning inside SGX enclaves. 
The library supports trusted domain applications conducting general computations. The library API encapsulates the data types of different access patterns. Internally, the library runs the application code in the following steps: Right before running into a TSX transaction, the library prepares the memory layout to be mapped to the CPU cache with a small footprint. When running inside the transaction, the library monitors CPU cache utilization by intercepting all memory references (captured through the encapsulated data types), accounting cache lines, and building a cache model with a small footprint in the CPU. Using the cache model, the library can predict which instruction will cause the next cache miss and lazily insert TSX instructions (e.g., \texttt{xend}) to declare the end of the transaction before it aborts. To predict cache misses in a controlled manner and reduce runtime overhead, we carefully engineer the library's memory layout and ensure the footprint of the cache model does not interfere with application data inside the CPU cache.

On top of the library, we implement a family of efficient data-oblivious algorithms (called external oblivious algorithms) to realize various data analytical computations in the enclave. 
Compared with classic ``word''-oblivious algorithms and ORAMs~\cite{DBLP:conf/ccs/StefanovDSFRYD13}, external oblivious algorithms have much lower time complexity and is also more promising for concrete performance efficiency. 
Specifically, external oblivious algorithms are a class of algorithms that accesses 1) an external data source, the access to which does not leak secret information, and 2) an internal ``stash'' that needs to be protected from leakage. We map an external oblivious algorithm to an enclave by placing the external data source outside hardware transactions and placing the code accessing the stash to run on our library inside transactions. 
These algorithms support various data analytics including sorting, shuffle, binary search, $K$-means, et al.
Altogether, the system achieves the notion of cache-miss obliviousness (i.e., the trace of cache misses during enclave execution is oblivious to the memory data being accessed) with provable security against most memory-access side-channels including the physical-level bus tapping.

We evaluate our library running external oblivious algorithm in two metrics: the transaction size and execution time. Specifically, we compare the transaction size resulted from dynamic partitioning with that from static partitioning (T-SGX) and manual partitioning schemes (Cloak). We also measure the execution time of running external-oblivious data analytical algorithms. We compare the execution time with that of word-oblivious algorithms (used in existing works, Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17}). The evaluation result shows that our work effectively increases the transaction size and reduces the execution time, both by orders of magnitude.

The contributions of this work are the following:

1. Proposed a new technique and built a library to dynamically partition the program and wrap the partitions in TSX transactions. The dynamic scheme works by monitoring cache utilization and ending a transaction when the CPU cache is almost full.

2. Develop a data-analytical system with strong side-channel security. The system runs external oblivious algorithms on top of the library inside SGX enclave.

3. Conducted performance evaluation that shows increased transaction size and reduced execution time by orders of magnitude in comparison with the state-of-the-art systems.




==> text/old/v2_approach.tex <==
\section{Research Formulation}

\noindent
{\bf Preliminary: TEE}. The architecture of SGX-alike TEE features a trusted world (a.k.a. enclave) and an untrusted world sharing a processor, the boundary between which is protected by some isolation mechanisms. The main memory usually resides in the untrusted world, where the content is protected by hardware encryption. 
In this TEE architecture, a memory reference has to access a series of micro-architectural ``buffers'', such as last-level cache (LLC), translation look-aside buffer (TLB), memory row buffer, etc., creating leakage side channels.

\subsection{System Model}
\label{sec:systemmodel}

\noindent
%{\bf System model}: 

In this work, we consider the modern computing paradigm that a security-sensitive computation is outsourced and run on a third-party host. This paradigm becomes increasingly popular due to the advent of cloud computing, which has cost-effectiveness, availability, etc. Concretely, the data owner possessing security-sensitive personal data uploads the data and program to a third-part host in the cloud where the program is executed over the data to evaluate the computation on the owner's behalf.

The host in our system has an SGX-alike trusted execution environment or enclave. The enclave is trusted by the data owner, including the processor at the hardware layer and the owner-provided program at the software layer. Hardware and software outside this perimeter of the enclave is untrusted by the data owner. 

\subsection{Threat Model}
\label{sec:threat}
This work considers memory-access pattern attacks in the emerging hardware enclaves. A program runs inside an enclave of a trusted processor and encrypted memory in the target system, and the adversary monitors a certain micro-architectural side-channel during the enclave execution. Based on the observed access trace, she then infers other sensitive information.
The exploited leakage channels include page-fault~\cite{DBLP:conf/sp/XuCP15}, page-table access/dirty bits~\cite{DBLP:conf/uss/0001SGKKP17,DBLP:conf/uss/BulckWKPS17}, cache-timing~\cite{DBLP:conf/ccs/WangCPZWBTG17,DBLP:conf/usenix/HahnelCP17}. 
Access-driven attacks against data-intensive computations can lead to significant information disclosure~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15,DBLP:conf/nsdi/ZhengDBPGS17,DBLP:journals/corr/BaterEEGKD16}.
For clarity, the non-goals of this work include other side-channel attacks (e.g., timing attacks, power analysis), denial-of-service attacks, rollback attacks, etc.

\subsection{Security Goals}
\label{sec:cmo}

Intuitively, the cache-miss obliviousness or CMO requires that the trace of cache-misses (as exposed in bus-tapping attacks) in a program execution should be independent of any execution data (both input and intermediate data). Consider executing a program $P$ with data $I$. The execution produces trace $T$ consisting of last-level cache misses. CMO requires that given two data values, $I_0$ and $I_1$, a CMO execution produces two identical traces, that is, $T_P(I_0)=T_P(I_1)$. 
This definition assumes that the computation induced by $P$ is deterministic. And the definition of obliviousness is ``perfect'' as it requires the two traces of different data are exactly the same.
We skip the more formal and generic definition of cache-miss obliviousness (e.g., based on indistinguishability formation~\cite{DBLP:books/crc/KatzLindell2007}). 

\subsection{Motivating Observation}
\label{sec:observation}

\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{figures/Executiontime-Transactionsize.eps}
%\includegraphics[width=0.35\textwidth]{figures/exp-Exectimeperinstruction-Transactionsize.eps}
%\includegraphics[width=0.35\textwidth]{figures/exp-Executiontime-Datasize.eps}
\caption{Preliminary performance observation with varying transaction sizes (with two arrays respectively of $64$ and $65536$ elements/cachelines).}
\label{exp:txsize:prel}
\end{figure}

This preliminary measurement study is designed to observe how the per-instruction execution time changes with the size of TSX transactions. We write a simple C++ program that writes to an array in a loop. Each array element has the same size with the cache line of the machine where the experiment is conducted. By this means, each access to an element can lead to a cache miss. The size of a transaction measures the number of instructions/iterations in the loop. Given a transaction size $t$, we wrap $t$ iterations in a TSX transaction by inserting \texttt{xend} and \texttt{xbegin}. We run the program with an array of 64 elements on an Intel SGX machine with the following specs: Intel(R) Core(TM) i5-7500 CPU @ 3.40GHz 64 bits, with 32 KB L1 cache size (8-way 64 sets) and 8 GB RAM. 
We consider two settings of array length: $64$ elements and $65536$ elements.
In the experiment, we vary the transaction size and report the average execution time per instruction over 1000 runs of the experiment. We also report the standard deviation.

The result in Figure~\ref{exp:txsize:prel} shows that the execution time generally decreases as transactions grow larger. Consider, first, the result with the $64$-element array.
When the transaction size increases from $8$ to $64$ iterations, the execution time decreases by $2\sim{}5\times$. This can be explained by that with larger transactions, the TSX transaction execution overhead (e.g., running \texttt{xbegin}/\texttt{xend} instructions and possible aborts) can be amortized to more instructions, leading to shorter execution time per instruction.
Note that transaction size $8$ is the maximal transaction size that can be set by a static scheme, such as T-SGX, on a CPU of $8$-way cache.

With the array of $64$ elements/cachelines, a transaction of maximal size would include all instructions updating the $64$ cachelines, does not cause cache misses and thus does not abort.
By contrast, this is not the case with the larger array of $65536$ elements/cachelines: A transaction of maximal size would cause cache misses and deterministically abort. As shown in Figure~\ref{exp:txsize:prel}, with the array of $65536$ elements, when the transaction is too large (e.g., 1024 loop iterations), it would incur very high overhead. Further when the transaction size is increased to $4096$ iterations, the transaction winds up in endless abort-re-execution and cannot complete. 

This preliminary study implies that while the transaction size resulted from static partitioning is too small and incurs high amortized overhead per instruction, enlarging transaction too much is not a good idea either. A proper transaction size that leads to good performance is the medium one, such as a transaction of $256$ iterations for an array of $65536$ elements in Figure~\ref{exp:txsize:prel}. In this work, we quantify this intuition by enlarging a TSX transaction until the next instruction to include would deterministically cause cache misses.

\section{Library for Dynamic Program Partitioning}

We design and develop a runtime system enforcing external data obliviousness inside SGX enclaves leveraging Intel TSX features.
Given a program expressing an external oblivious algorithm, the system provides an API (S1) for developers to annotate the leaky section of the program. Given the annotated program, we provide an execution engine (S2) that runs the program on the architecture of two execution environments: the one with access-pattern protection (e.g., prohibiting cache-misses) and the other without. We call the former by fortified enclave and the latter by unprotected enclave. Briefly, the execution engine partitions the runtime instance dynamically in a way that assures no cache-miss yet can scale to relatively large data.
Figure~\ref{fig:overview} illustrates the overview of our system. In the following, we present the detailed design and implementation of our system in each component, S1 in \S~\ref{sec:api} and S2 in \S~\ref{sec:dynpart}.

\begin{figure} 
\centering
%\includegraphics[width=0.26\textwidth]{figures/system-overview.eps}
\includegraphics[width=0.225\textwidth]{figures/figure1.eps}
\caption{System overview: A target computation is annotated by our programming API that specifies data-access pattern. Our runtime system first partitions the program dynamically to units (i.e., dynamic partitioning), and then runs each unit in a TSX transaction (i.e., tx-execution engine).}
\label{fig:overview}
\end{figure}

\subsection{Annotating Target Programs}
\noindent
\label{sec:api}

%{\bf API}: 
Our system provides a programming interface for C++ developers to annotate the leaky section of the program and define the type of data referenced inside the leaky section. Specifically, 1) we provide two library functions, \texttt{begin\_leaky()} and \texttt{end\_leaky()}, for developers to declare the begin and end of a program snippet where leaky memory access occurs. 2) In addition, all the memory data accessed inside a leaky section needs to be defined with our data type. We provide four data-container types as defined below. The explicit data type allows our execution engine to know ahead of time the possible data-access pattern and take action in partitioning more precisely.

The data-container types are classified based on whether the access is leaky and whether the data is read-only. The four data types are \texttt{NobRO}, \texttt{ObRO}, \texttt{NobRW}, \texttt{ObRW}, where \texttt{ObRW} stands for oblivious read-write data container and NobRO is non-oblivious read-only data container. The API of the data classes are provided in Figure~\ref{lst:samplecode}. We also provide an example code that declares the merge passes in a merge sort algorithm to be leaky sections.

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
class ObRO {
  int32_t read_next(); 
  void reset();
}
class ObRW {
  void write_next(int32_t data); 
  void reset();
}
class NobRW {
  int32_t read_at(int32_t addr);
  void write_at(int32_t addr, int32_t data); 
}
class NobRO {
  int32_t nob_read_at(int32_t addr); 
}
\end{lstlisting}
\end{minipage}
\\
\vspace{-0.35in}
\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
void MergeSort(int[] array, int start, int end){ 
  if (start == end - 1) return;
  MergeSort(array, start, (end + start)/2); 
  MergeSort(array, (end + start)/2, end);
  Merge(array, 0, (end + start)/2, (end + start)/2, end);
}
void Merge(int[] array, int start1, int end1, int start2, int end2){
  *NobRW* parray = new *NobRW*(array);
  *begin_leaky();*
  originalMerge(parray, start1, end1, start2, end2); 
  *end_leaky();*
}
\end{lstlisting}
\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Implementing merge sort based on the CMO API: in-transaction data types and leaky section}
\label{lst:samplecode}
\end{figure}

\subsection{Realizing Dynamic Program Partitioning}
\label{sec:dynpart}

\noindent{\bf Design motivation}:
Existing side-channel defenses leverage the hardware transaction features to detect any unintended cache misses. Notably, Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} detects cache attacks using Intel TSX. Briefly, it executes the computation in HTM transactions, such that the intra-transaction memory accesses are resolved by cache hits and thus are concealed from the adversary. Note that the inter-transaction memory accesses are disclosed. The security of these Cloak alike schemes requires that access-leaky memory regions must reside in data cache; this security requirement significantly limits the data scale. In addition, Cloak's programming interface is rather low-level and requires the programmer to manually specify the scope of individual HTM transactions, which further limits its applicability in big-data computations.

To systematically improve the data scalability, we study two technical problems: (O1) dynamic program partitioning and (O2) enlarging transaction. First, given a target computation, we dynamically partition the program to smaller execution units, each run in an individual transaction. Compared with existing work, such as Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} and T-SGX~\cite{shih2017t}, our unique perspective about program partitioning is to take into account various runtime information (see \S~\ref{sec:approach} for detailed comparison). 

Second, for each execution unit, we enlarge the transaction as much as possible. Here, the larger a transaction is, the more performance efficient it can be, as the transaction setup cost (e.g., running \texttt{xbegin}/\texttt{xend} instructions) can be amortized among more instructions. Note that the size of any TSX transaction has a theoretic limit in that its working set cannot exceed a CPU data cache. Our goal is to reach this theoretic bound in transaction size. 

\noindent{\bf 
Design rationale}: 
As revealed in our API design in \S~\ref{sec:api}, a starting point of our approach is to expose to the runtime system some high-level semantic information. This information includes different types of data accesses; concretely, the data-container types in our API lets the runtime be aware of four data-access classes: 1) non-oblivious reads (or access-leaky reads as in \texttt{NobRO}), 2) non-oblivious writes (or access-leaky writes as in \texttt{NobRW}), 3) oblivious reads (as in \texttt{ObRO}) and 4) oblivious writes (as in \texttt{ObRW}). 

With awareness of data access type, we can specify the constraints of program partitioning problem. In general, there are two constraints, the constraint imposed by the TSX hardware (C1) and that imposed by the security requirement (C2). 
Figure~\ref{fig:constraints} illustrates the two constraints in the presence of four types of data accesses. 
For C1, it requires that a transaction's write-set should not cause L1 cache replacement, and a transaction's read-set should not cause LLC cache replacement. For C2, the access-leaky memory region must reside in data cache without being split.  Here, an access-leaky memory region is defined by memory data accessed in a data-dependent way; for instance, \texttt{NobRO} and \texttt{NobRW} instances are access-leaky regions.\footnote{We may use terms \texttt{NobXX} to represent access-leaky regions} The constraint of C2 is due to the strong security concern. Because the HTM based protection only conceals the intra-transaction memory access pattern, and the inter-transaction memory access pattern is disclosed. Placing the leaky memory accesses across multiple transactions would inevitably disclose the data secrets. 

\begin{figure} 
\centering
\includegraphics[width=0.35\textwidth]{figures/constraints.eps}
\caption{Transactional data constraints imposed by hardware (C1) and security (C2) requirements. The data is classified to four types based on read/write and leaky/non-leaky.} 
\label{fig:constraints} 
\end{figure}

Because of the constraints (particularly C2), we focus on {\it partitioning the non-leaky part of the program}. That is, we consider the problem of partitioning the program into smaller units, each unit accessing a partition of non-leaky data (\texttt{ObXX}) but accessing leaky data in their entirety. Note that the leaky data is not partitioned and has to be loaded in total to the data cache. This design choice implies that we only support computation with small cache-bound leaky data (\texttt{NobXX}).\footnote{Note that the assumption presents a fundamental limitation of our approach in supporting computation of large access-leaky data.}, which is consistent with our target computations (as described in \S~\ref{sec:computation}).  

Our goal is two-fold: (O1) Support computations of (non-leaky) data as large as possible by dynamically partitioning the computations, 
and (O2) Run these computations using transactions of as large size as possible.

The high-level approach is illustrated in Figure~\ref{fig:shadow}. As in the figure, consider a computation whose application memory consists of (cache-bound) access-leaky data (i.e., A1 and A2) and large non-leaky data (i.e., A3 and A4). We split the non-leaky data into a series of smaller data partitions (i.e., \{P3\} and \{P4\}), each of which is small enough to fit in a CPU data cache. 
To support large transactions (O2), we enable {\it L1 cache replacement on read-only data}. That is, the footprint of A1 and P3 in L1 cache can be reduced to just one set, as will be explained next.

\fbox{\parbox{0.90\linewidth}{
Formally, our work can be formulated as an optimization problem: Given a program $G$ on data $\{A1,A2,A3,A4\}$, it partitions $G$ to a series of $\{g\}$ with each program partition $g$ operate on data $A1,A2,P3,P4$ such that it maximizes $\min{(P3,P4)}$ and it is subject to the following constraints:

\begin{eqnarray}
  \nonumber
\cup\{P3\} & = & A3\\
  \nonumber
\cup\{P4\} & = & A4\\
  \nonumber
A1 + P3 + A2 + P4 & < & LLC\\
  \nonumber
A1/L + P3/L + A2 + P4 & < & L1
\end{eqnarray}

Here, $L$ is the maximal number of LLC cache lines that can be mapped to one L1 cache set.
}}


\label{sec:shadowmem}
\noindent
{\bf Large transactions by shadow memory}:
As will be described next, read-only data (A1 and P3) in a transaction can reuse L1 data cache without aborting the transaction. 

%cache full utilization is essential.\footnote{For instance, a poorly utilized cache may abort a transaction when just one set (out of say 64 cache sets) is full. A well-utilized cache may abort a transaction when the entire cache is full, which results in a much larger transaction.} 

Efficient use of the cache is of particular importance to ensuring large transactions. The transaction will not abort when the cache is underutilized; for instance, the transaction may end when only one cache set (out of 64) becomes full while the other sets are empty.

We propose a technique called shadow memory that arranges the in- transaction memory layout such that memory data is mapped to the CPU cache hierarchy without unnecessary conflict. Briefly, we enforce the rules that different types of data (A1, ...A4) should not overlap in data caches. Specifically, consider a cache hierarchy with a 8-way 32KB L1 cache and 16-way 8MB L2 cache. We allocate $60$ L1C sets to be A2 (\texttt{NobRW}), $2$ L1C sets to be P4, $1$ L1C set to be P3 and $1$ L1C set to be A1. Note that A1 and P3 can reuse the L1 cache and their sizes are bounded by LLC. Figure~\ref{fig:shadow} illustrates an example of shadow memory.

\begin{figure} 
  \centering
%  \includegraphics[width=0.475\textwidth]{figures/shadow_memory_cache.eps} 
  \includegraphics[width=0.475\textwidth]{figures/figure4.eps} 
  \caption{Splitting data to transaction-wise partitions and mapping data to the memory/cache hierarchy: Shadow-memory is an indirection layer that arranges data in cache based on the access pattern. From LL (Last-Level) cache to L1 (Level-one) cache, read-only data replacement is enabled. In the figure, A1 (A2) represents the read-only (read-write) data whose access pattern leaks sensitive information, and A3/P3 (A4/P4) represents the read-only (read-write) data whose access pattern does not leak sensitive information.} 
\label{fig:shadow} 
\end{figure}

\noindent
{\bf Implementation notes}:
When realizing the dynamic partitioning, we encountered two design problems: 1) How and when to insert the \texttt{xbegin} and \texttt{xend} instructions to properly declare transaction boundaries such that the transactions can successfully finish their execution (i.e., without abort) yet are not prematurely ended? 2) How to realize the shadow memory in its full life cycle? 3) How to decide the condition that the computation cannot be executed using transactions at an early time (e.g., when the A1 is larger than LLC).

We build a library that realizes the partitioning life cycle. Recall that our API supports declaring the leak section's scope and wrapping each in-transaction memory access by custom data types. Upon leaky section declaration, we realize the allocation of shadow memory. Upon the in-transaction memory access, we hook the transaction partitioning schemes. The overall mechanism is illustrated in Figure~\ref{fig:libimpl}, and pseudo-code is presented in Listing~\ref{lst:samplecode:hook}.

\begin{figure} 
  \centering
  %\includegraphics[width=0.4\textwidth]{figures/lib_impl.eps}
  \includegraphics[width=0.4\textwidth]{figures/figure5.eps}
\caption{Library implementation: Each box represents a function in our library. White boxes run outside TSX transactions and blue boxes run inside TSX transactions.} 
\label{fig:libimpl} 
\end{figure}

Concretely, for shadow memory allocation, we allocate the shadow memory according to the layout described in \S~\ref{sec:shadowmem}. Note that the shadow-memory size is fixed (as the total size of a cache is fixed). We perform checks on whether the data size, specifically the size of access-leaky memory data, is small enough to fit into the data cache. In other words, we enforce the constraint C1 that A1 does not exceed L1 and A2 does not exceed LLC.

For transaction partitioning, we implement two components: 1) monitoring cache usage, and 2) realizing transaction partitioning. For 1), we simply monitor the condition that if each non-leaky data overflows, that is, the iterator call to \texttt{ObXX.next()}\footnote{\texttt{ObXX} refers to non-leaky data type, either \texttt{ObRO} or \texttt{ObRW}.} reaches its full capability. Note that we enforce a joint capability limit, that is, the total size of \texttt{ObXX} objects is bounded instead of individual \texttt{ObXX}.

For 2), we insert the TSX instructions \texttt{xend} and \texttt{xbegin}. Between them, we make data copy between shadow memory and application memory of the non-leaky data. Because the computation is partitioned based on non-leaky data, different transactions in the same leaky-section computation will use different non-leaky data, thus making it necessary to reload non-leaky data across transactions. Also, we preload data twice across transactional boundary.

\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  caption={Library implementation: Hook partitioning triggers in non-leaky data scans.},                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  label={lst:samplecode:hook},
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
begin_leaky(){
  shadow_memory_alloc();
}
//Dynamically partition computations in next();
ObXX::next(){
  //1. monitor the overflow
  if(shadow_mem.ob.size + 1 < shadow_mem.ob.capability()) return;
  //2. start to partition
  if(!first_time) xend();
  //reload non-leaky data (ob) in shadow memory from application memory
  shadow_mem.reload_ob();
  double_preload();
  xbegin();
}
\end{lstlisting}

\section{The Case of Cache-miss Oblivious Data Analytics}
\label{sec:cases}
\label{sec:computation}

While our library supports generic computation, we use it to implement the external-oblivious algorithms as a prototype system of secure data analytics.
We first present the preliminary of external oblivious algorithms and then describe how to implement them using our library.

\subsection{Preliminary: External Data-Oblivious Algorithms}
\label{sec:prel:externalobl}

External data-oblivious algorithms are a class of oblivious mechanisms that have advantageous time complexity at the expense of assuming a trusted internal memory or so-called ``stash''. External oblivious algorithms are proposed for a wide variety of computations, including shuffle (Melbourne shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14}), sort (oblivious merge sort~\cite{DBLP:conf/ndss/WilliamsS08}), most aggregation computations, etc. Compared with word-oblivious algorithms (e.g., sorting networks causing a multiplicative factor of $O(\log{N})$), an external oblivious algorithm has better time complexity (e.g., Melbourne shuffle based sorting~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15,DBLP:journals/popets/DangDCO17} with the O(1) multiplicative factor). Compared with ORAM (with a multiplicative factor of $O(\log^2{N})$), an external oblivious algorithm is specific to target computation and is more efficient.
While external oblivious algorithms achieve better complexity, they may present limitations on data scalability. Concretely, most existing external oblivious algorithms are designed for a client-server setting and assume a large internal memory at the client side. For instance, a Melbourne shuffle assumes an internal memory of $O(\sqrt{N})$. The large internal memory may be suited for a client machine (in the big-data setting), but presents challenges when treating cache as internal memory, whose size is very limited; for instance, a L1 cache is 32 KB and L3 cache is 8 MB in an Intel SGX CPU. Very recently, space-efficient external oblivious algorithms are proposed, for instance, stash shuffle with small $O(\log{N})$ internal space.

\subsection{Implementing External Oblivious Data Analytics}

Here, we present our experience building various external-oblivious computations using our library. 

\noindent{\bf $K$-means}:
A $K$-means computation takes as input a data array and randomly initialized K centroids. It produces the output of K centroids in K clusters that are the most representative of the data array. Here, each element in the data array represents a data point, and there are pair-wise distances defined between them. The $K$-means computation runs iteratively, where each iteration consists of two data passes, one (KM1) is a nested loop that (re)-assigns every array element to the closest centroid, and the other (KM2) is an array scan that randomly accesses the centroid array to update the centroid position. 

K-means is an external oblivious computation in the sense that it keeps the centroid as internal memory accessed in a leaky way and the data array as an external memory, which is accessed obliviously. 

To implement $K$-means using our library, we declare the data pass (KM2) to be the leaky section where the internal memory is accessed. In the leaky section, the centroid array is defined as a NobRW, data array as an \texttt{ObRO}, the data-centroid mapping as an \texttt{ObRW}. 
%The related sample code is in Listing~\ref{XXX}.

\begin{figure*}[!tbhp]
\centering
\subfloat[Binary search: Number of queries]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofqueries.eps}
  \label{exp:bs:query}
}
\subfloat[Binary search: Number of records]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-binarysearch.eps}
  \label{exp:bs:data}
}
\subfloat[$K$-means: Number of records]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-kmeans.eps}
  \label{exp:kmeans:data}
}
\subfloat[$K$-means: Number of centroids (K)]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Valueofk.eps}
  \label{exp:kmeans:k}
}
\caption{Comparing CMO with scan: Binary searches and k-means}
\label{exp:vsscan}
\end{figure*}



\noindent{\bf Melbourne shuffle}:
A Melbourne shuffle is a randomized algorithm for data shuffling. A data-shuffle operation takes as input two arrays of equal length, one storing data and the other storing a permutation. It produces the output of permuted data array. For instance, $\texttt{mshuffle}({x,y,z},{1,0,2})={y,x,z}$. Internally, Melbourne shuffle is a randomized algorithm that bucketizes each of the two arrays to $\sqrt{N}$ buckets, each of $\sqrt{N}$ size. A Melbourne shuffle runs in two rounds, each round using $\log{N}\sqrt{N}$ internal memory accessed in a leaky fashion. The original input arrays are in external memory.

To implement Melbourne shuffle using our library, we declare both rounds to be leaky sections. In particular, for scalability, we declare the first round, which is to ``distribute data bucket based on permutation bucket'', to be two leaky sections. Briefly, the first leaky section in the distribution round produces the unordered, linked list as output, without dummy elements. The second leaky section adds dummy elements. In this way, we can improve the data scalability significantly and reduce the access-leaky internal memory from $O(\log{N}\sqrt{N})$ to $O(\sqrt{N})$.   

\noindent{\bf Oblivious merge sort}:
In oblivious merge sort, the operation of merging two sorted lists is made oblivious by a randomized algorithm~\cite{DBLP:conf/ndss/WilliamsS08}. Given two sorted lists, an oblivious merge keeps a $O(\sqrt{N})$ internal-memory buffer and finishes the merge computation with the same $O(N)$ complexity. It is a randomized algorithm and the probability of internal buffer overflowing is made negligible.  

We implement oblivious merge sort by declaring the merge operation to be a leaky section and the internal buffer to be a \texttt{NobRW} and the two merging arrays to be two \texttt{ObRO}.

\noindent{\bf 
Streaming binary search}:
Consider a query on a sorted data array. A binary search locates the matching element in the array to the query. Given a stream of queries, the binary search can be treated as an external-oblivious process in the sense that the internal memory maintains the data array, and external memory maintains the query stream.

To implement the streaming binary search using our library, we declare the binary search to be the leaky section, the data array to be a \texttt{NobRO}, the query stream (array) to be an \texttt{ObRO}. 

\section{Performance Evaluation}

This section evaluates the performance of our system under different sizes of datasets (data scalability). 

%\subsection{Macro Benchmark}

\noindent{\bf Comparison with scan baseline}: 
This set of experiments evaluates the performance of CMO, in comparison to scan-based baselines.  The scan-based baseline translates each leaky random access (on \texttt{NobXX}) to a full array scan. Note that while ORAM~\cite{DBLP:conf/ccs/StefanovDSFRYD13,DBLP:journals/jacm/GoldreichO96} presents a generic solution with better (asymptotic) efficiency, the scan-based approach is state-of-the-art and is more frequently chosen for in-memory data processing, such as oblivious machine learning~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16} and ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}\footnote{ZeroTrace uses ORAM for disk data access and scan for its internal-memory data access.}. In addition, at a medium data scale, the better asymptotic efficiency of ORAM may not translate to better concrete performance. We implement the scan baseline in our library by converting each access to \texttt{NobXX} to a full-array scan.

We consider the various data analytical computations in the experiments. In each experiment, we measure the performance by execution time. Specifically, the execution time only includes the time spent on running the computation and excludes the time spent on initial data loading (to the cache). We use numeric datasets and generate them randomly. 

We did all the experiments on a laptop with an Intel 8-core i7-6820HK CPU of 2.70GHz, 32KB L1 and 8MB LL cache, 32 GB RAM, and 1 TB Disk. This is one of the Skylake CPUs equipped with both SGX and TSX features. 

\begin{figure}
\subfloat[Melbourne shuffle]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-melbourne.eps}
  \label{exp:melbourne:data}
}
\subfloat[Oblivious merge sort]{%
  \includegraphics[width=0.25\textwidth]{figures/exp-Executiontime-Numberofrecords-mergesort.eps}
  \label{exp:oms:data}
}
\caption{Comparing CMO with scan: External-oblivious sorts}
\label{exp:vsscan2}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/exp-Executiontime-Numberofrecords-sorting.eps}
\caption{Comparing CMO with word-obliviousness and Cloak: the case of sorting}
\label{exp:sorting}
\end{figure}


We vary the data size in each computation and report the results in Figures~\ref{exp:vsscan} and ~\ref{exp:vsscan2}. 
Figure~\ref{exp:melbourne:data} and ~\ref{exp:oms:data} evaluate the execution time of Melbourne shuffle and oblivious merge sort. Compared with the baseline of scan approach, the Melbourne shuffle by CMO achieves a speedup of more than $100\times$ at the largest data scale of 1 million records. For oblivious merge sort, the speedup is much less significant, about $10\%$ speedup of the baseline. 
%The reduced speedup is related to the fact that XXX. 

Figures~\ref{exp:bs:data} and~\ref{exp:bs:query} present the performance result of streaming binary search with varying data size and the number of queries. With varying data size, the CMO outperforms the scan baseline by a speedup ranging from $100\times$ to $1000\times$. With varying query numbers, CMO first keeps the execution time constant until the cache cannot accommodate all the queries. CMO's execution time then linearly scales with the query number. With a large query number, CMO outperforms the scan baseline by $1000\times$ times. Similarly, the performance result of $K$-means in Figures~\ref{exp:kmeans:data} and~\ref{exp:kmeans:k} also show multi-magnitude speedup of CMO.

\noindent{\bf Comparison with other algorithms}:
This set of experiments is to evaluate the performance of CMO against two baselines: 1) word-oblivious algorithms without any TSX transactions, and 2) TSX transactions with no automatic partitioning (e.g., in Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}). For fair comparison, we consider the computation task of sorting and require all approaches achieve the same security level, that is, cache-miss obliviousness. Under this setting, different approaches may run different sorting algorithms. For instance, for 1), the chosen algorithms have to be word oblivious, and we use bubble sort in this baseline. For 2), the algorithms do not need to be oblivious (as the side-channels are defended against by TSX transactions). Thus, we choose the more efficient algorithms, the quick sort. For our work, we use three external oblivious sorting algorithms: Melbourne shuffle with quick sort (following the scramble-then-compute paradigm~\cite{DBLP:journals/popets/DangDCO17}), oblivious merge sort, and cache shuffle with quick-sort. 

The performance result is presented in Figure~\ref{exp:sorting}. The ideal baseline of quick sort running with TSX transactions can only scale to 1024 data records. Because this approach does not partition the program and their computations' working set is limited to the size of CPU cache.
Our CMO approach running oblivious merge sort is limited to support data size of $2^{14}$ records due to the large ``stash'' in the oblivious merge sort algorithm. The other approaches including CMO running Melbourne and cache shuffles, as well as the baseline of word-oblivious bubble sort can scale to large datasets.
In terms of execution time, the CMO approach achieves a speedup by up to two orders of magnitude compared with the word-oblivious bubble sorts (without TSX transactions). This speedup is especially obvious when the data size is more than $2^{14}$ records.

\section{Related Work}

\subsection{Memory-Access Side-Channel Attacks}
\label{sec:background}
\noindent
{\bf Memory-access attacks}: A passive memory-access attacker monitors the access trace of an enclave execution and infers sensitive information. To monitor, the attacker {\it breaks} enclave execution and {\it observes} some micro-architectural side-channel. 
Existing memory-access attacks can be characterized by the spatial resolution of the leakage channel being observed and the temporal resolution of breaking the enclave control flow.
For instance, in the seminal work~\cite{DBLP:conf/sp/XuCP15}, 
a controlled page-fault attacker observes and breaks the enclave execution through page-fault interrupts, where the trace' spatial granularity is page numbers and the temporal granularity is individual page accesses. 
More advanced attacks exploit other leakage channels (e.g., page-table access/dirty bits~\cite{DBLP:conf/uss/BulckWKPS17,DBLP:conf/ccs/WangCPZWBTG17}, shared last-level caches~\cite{DBLP:conf/usenix/HahnelCP17}) to improve spatial and temporal resolution. 
To make it harder to defend against, recent {\it stealthy} attacks break the enclave execution invisibly through hyper-threading that
eliminates interrupts~\cite{DBLP:conf/uss/GrussLSOHC17,DBLP:conf/ccs/WangCPZWBTG17}. 

\ignore{
\begin{figure}
\begin{center}
  \includegraphics[width=0.35\textwidth]{figures/sgxattacks-def.eps}
\caption{Taxonomy of memory-access attacks and defenses in SGX: {\small
Existing attacks shown in the diagram are code-named by the publication venue and year, including USS17 (USENIX Security)~\cite{DBLP:conf/uss/BulckWKPS17}, CCS17~\cite{DBLP:conf/ccs/WangCPZWBTG17}, SysTex17~\cite{DBLP:conf/sosp/BulckPS17}, ATC17~\cite{DBLP:conf/usenix/HahnelCP17}, OAKLAND15~\cite{DBLP:conf/sp/XuCP15}. Existing defenses shown in the diagram are code-named similarly and with their name, including T-SGX~\cite{shih2017t}, D\'ej\`a Vu~\cite{DBLP:conf/ccs/ChenZRZ17}, and Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}.
}}
\label{fig:sgxattacks}
\end{center}
\end{figure}
}

\subsection{Attack Mitigation by Isolation}

\noindent
{\bf Memory-access attack mitigation}:
A successful memory-access attack entails two conditions: 1) an observable channel of memory-access leakage, and 2) the capability of relating the leaked memory-access to sensitive information. A memory-access attack can be mitigated by breaking either condition: M1) Detecting that a leakage channel is being observed by {\it enclave fortification}, or M2) Eliminating the source of leakage by making it difficult to correlate the access trace with sensitive information, via {\it obliviousness}. 

{\color{black}
Existing mitigation techniques take different views regarding how side-channel attack works and takes action to close the leakage channel (i.e., isolation). SGX-LAPD~\cite{DBLP:conf/raid/FuBQL17} mitigates the page-fault attacks by enforcing that OS uses large pages. This property  of untrusted OS is verified by the enclave running a program to test the time of page fault. 

T-SGX~\cite{shih2017t} closes the page-fault channel by preventing interrupts in enclaves leveraging the TSX capability. Specifically, by wrapping computation into TSX transactions, any interrupt, including page faults that occur inside a transaction, will be captured by the software. T-SGX runs a policy that bounds the number of interrupts/page-faults to prevent page-fault attacks.

Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} and the work from Chen, et al~\cite{DBLP:conf/ccs/ChenLMZLCW18} close the cache side channels by detecting (individual) cache misses using TSX transactions.

Varys~\cite{DBLP:conf/usenix/OleksenkoTKSF18} reduces all existing side-channel attacks to two leakage channels, namely SGX's Asynchronous EXit (AEX) events and concurrent sharing of CPU cores. To close the first channel, it proposes to monitor the enclave AEX and terminate the enclave execution when the AEX frequency exceeds a threshold. It allocates sufficient hyperthreads to keep a CPU core occupied by a single application (so-called thread-core reservation) to close the second channel. Vary enforces the two conditions (AEX monitoring and thread-core reservation) in a trust-but-verify manner, that is, the OS is trusted to execute the program with the required property verified nevertheless by the enclave.
}

For the former, existing enclave-fortification work detects the attack on the events of page-fault~\cite{DBLP:conf/ccs/ShindeCNS16,shih2017t}, cache-miss~\cite{DBLP:conf/uss/GrussLSOHC17,DBLP:conf/woot/BrasserMDKCS17}, etc. 

For the latter, existing work on {\bf data-oblivious systems} is based on oblivious algorithms~\cite{DBLP:conf/nsdi/ZhengDBPGS17,DBLP:conf/ccs/OhrimenkoCFGKS15} or less-efficient oblivious RAM~\cite{DBLP:journals/iacr/SasyGF17,2017arXiv171000458E}.
Concretely, data obliviousness can eliminate the source of leakage in the presence of memory-access attacks on TEE. When building data-oblivious systems, a design choice is which oblivious-computing mechanisms to use: Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17} supports database queries by engineering word-oblivious algorithms (Column Sort~\cite{DBLP:journals/siamcomp/AzarV87}). Oblivious machine-learning~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16} combines word-oblivious algorithms and the trivial mechanism of converting random-access to a full-array scan. Scan-based transformation is similarly adopted in building ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}, an ORAM system in SGX. ObliVM~\cite{DBLP:conf/sp/LiuWNHS15} is a compiler that supports the engineering of both word-oblivious algorithms and ORAM~\cite{DBLP:conf/ccs/StefanovDSFRYD13,DBLP:journals/jacm/GoldreichO96}. Oblivious Map-Reduce~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15} and Prochlo~\cite{DBLP:conf/sosp/BittauEMMRLRKTS17} use external oblivious shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14} to protect distributed systems under traffic analysis, but insecure under micro-architectural memory-access attacks. 

\subsection{Attack Mitigation by Data Obliviousness}

\noindent
{\bf Data-oblivious algorithms}:  The conventional oblivious algorithms ensure oblivious data access at the ``word'' granularity. These {\it word-oblivious algorithms (A1)} are constructed based on primitives such as compare-exchanges and tend to be not very practical (e.g., AKS sorting~\cite{DBLP:conf/stoc/AjtaiKS83} and sub-optimal column sort~\cite{DBLP:journals/siamcomp/AzarV87}). In the external-memory model, {\bf external oblivious algorithms} improve the time/IO complexity by assuming a small amount of internal storage that is accessed in a leaky fashion. Due to a smaller constant and optimal complexity, this family of algorithms is of great practical interest. For instance,  Melbourne shuffle~\cite{DBLP:conf/icalp/OhrimenkoGTU14} causes $O(\sqrt{N})$ IO with $O(N\log{N})$ time at the expense of $\sqrt{N}$ internal space and was recently used in constructing practical systems (e.g., MapReduce~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15}). Research to improve the algorithmic ``locality'' and to further reduce the internal-space complexity is underway~\cite{DBLP:journals/corr/abs-1709-07553}. The {\it oblivious RAM (A3)}~\cite{DBLP:conf/ccs/StefanovDSFRYD13,DBLP:journals/jacm/GoldreichO96} is an external data structure supporting oblivious external data access by translating virtual random-access to oblivious physical data access with poly-logarithmic blowup.

Compared with ORAM (A3) and word-oblivious algorithms (A1), the external oblivious algorithms (A2) cause lower overhead in complexity. Compared with generic ORAM, external oblivious algorithms are computation specific; existing algorithms support sort, compaction, and relational queries and other batched-oriented computations~\cite{DBLP:conf/icalp/OhrimenkoGTU14,DBLP:conf/ndss/WilliamsS08,DBLP:conf/spaa/Goodrich11,DBLP:conf/icdt/ArasuK14}.

\ignore{
\begin{table*}[!htbp] 
\caption{Research distinction}
\label{tab:distinct}\centering{
\small
\begin{tabularx}{0.9\textwidth}{|c|c|X|X|X|}
  \hline
 & Method
 & Cache access-pattern security 
 & Data scalability 
 & Algorithmic complexity \\ \hline
  T-SGX~\cite{shih2017t}, Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}
  & Attack detection by HTM & + & - & + \\ \hline
  Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17}, ObliviousML~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16}
  & Word-oblivious algo. & + & + & - \\ \hline
  ObliviousMR~\cite{DBLP:conf/ccs/OhrimenkoCFGKS15},Prochlo~\cite{DBLP:conf/sosp/BittauEMMRLRKTS17}
  & External oblivious algo. & - & + & + \\ \hline
  ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17}
  & External ORAM & + & + & - \\ \hline
  This work
  & External oblivious algo./HTM & + & + & + \\ \hline
\end{tabularx}
}
\end{table*}
}

\section{Conclusion}
This work enables cache-miss oblivious data analytics with Intel SGX. It considers expressing target data analytics by external oblivious algorithms and protects their stash's memory access pattern by dynamically partitioning the code and wrapping them in TSX transactions. 
We develop a C++ library that monitors  memory accesses and builds a cache model to predict cache misses. 
On the library, we implement various external oblivious algorithms.
The evaluation shows effectively increased transaction size and reduced execution time by orders of magnitude in comparison with the state-of-the-art systems.


==> text/old/v2_intro.tex <==
\section{Introduction}
In today's trusted execution environments (TEE), notably Intel SGX, memory content is encrypted with the intent to protect data confidentiality against a privileged adversary (e.g., a malicious operating system).
However, recent practical attacks on SGX have demonstrated the feasibility of extracting the plaintext of memory content by observing only the memory access pattern disclosed through various micro-architectural side channels (e.g., page fault, cache timing, etc.~\cite{DBLP:conf/sp/XuCP15,DBLP:conf/uss/BulckWKPS17,DBLP:conf/uss/0001SGKKP17,DBLP:conf/ccs/WangCPZWBTG17}). Protecting memory access pattern against such side-channels becomes the last defense and is critical to the overall TEE security.

The software-only defense has innate advantages in deployability on off-the-shelf TEEs. A practical software-only defense entails three relevant features: 1) security which defines how effective the defensive mechanism is to mitigate various side-channel attacks and to preserve data confidentiality, 2) data scalability which defines how big the dataset is that the defensive system can scale up to, and 3) performance overhead which defines the performance slowdown caused by the defensive mechanism.

This work follows a promising general approach that repurposes Intel's hardware transactional memory feature (TSX) for side-channel protection. Briefly, TSX allows executing programs in hardware transactions that are bound to abort with control returned to software if a cache miss occurs inside the transaction.
Thus, successful completion of a TSX transaction implies no occurrence of cache misses and thus no chance to leak memory access patterns outside the trusted CPU. 

Existing research works~\cite{shih2017t,DBLP:conf/uss/GrussLSOHC17,DBLP:conf/ccs/ChenZRZ17} follow this TSX-based hardening approach and focus on the design problem of wrapping target programs in TSX transactions.
Specifically, Cloak~\cite{DBLP:conf/uss/GrussLSOHC17} and D\'ej\`a Vu~\cite{DBLP:conf/ccs/ChenZRZ17} defend against cache-timing attacks and consider only protecting cryptographic libraries where a typical procedure has a small, cache-resident working set and can be directly mapped to a TSX transaction. These two works achieve security but incur high overhead with limited data scalability, as summarized in Table~\ref{tab:distinction}.
To support generic computations where a procedure's working set is commonly much larger than a CPU cache, T-SGX~\cite{shih2017t} partitions a target computation at the compilation time (as an LLVM extension) into pieces, each of which has a working set small enough to fit into the cache and can be run inside a TSX transaction.
As a static scheme, T-SGX has to consider the worst-case at runtime and make each program partition conservatively small to avoid (deterministic) transaction aborts. For instance, on a $8$-way cache, each program partition from T-SGX should have no more than $8$ memory instructions. Otherwise, there is a chance that a transaction would request more memory accesses than a cache line of $8$ slots, which makes a conflict cache miss bound to happen and the transaction bound to abort.
Thus, transactions induced from T-SGX or, more generally, from a static partitioning scheme,
are rather small, which leads to degraded security and performance overhead, as will be explained next. T-SGX's design tradeoff is depicted in Table~\ref{tab:distinction} where
\cmark\kern-1.1ex\raisebox{.7ex}{\rotatebox[origin=c]{125}{--}} means T-SGX defends against certain attacks (page-fault controlled side-channels~\cite{DBLP:conf/sp/XuCP15}) but not other attacks, such as cache-timing based side-channel.

\begin{table}[!htbp] %force in current page, disable float.
\caption{Existing hardening works based on TSX and the distinction of this work.}
\label{tab:distinction}\centering{\footnotesize
\begin{tabularx}{0.5\textwidth}{ |c|X|X|l|l|l| }
  \hline
Systems & Partitioning method & Scalability & Security against cache timing & Security against page faults & Perf.
  \\ \hline
Cloak~\cite{DBLP:conf/uss/GrussLSOHC17}
& 
\multirow{2}{*}{Manual} 
&
\multirow{2}{*}{\xmark} 
& 
\multirow{2}{*}{\cmark} %(Cache-timing attacks only)
& \multirow{2}{*}{\xmark} %(Cache-timing attacks only)
& \multirow{2}{*}{\xmark}
  \\ \cline{1-1}
D\'ej\`a Vu~\cite{DBLP:conf/ccs/ChenZRZ17} 
& & & & \\ \hline
T-SGX~\cite{shih2017t} & Static & \cmark  & 
%\cmark\kern-1.1ex\raisebox{.7ex}{\rotatebox[origin=c]{125}{--}} %(Page-fault attacks only) 
\cmark & \xmark & \xmark
  \\ \hline
This work & Dynamic & \cmark & \cmark & \cmark & \cmark
  \\ \hline
\end{tabularx}
}
\end{table}

This work aims at scaling TSX-based hardening schemes to support generic computations with strong security against memory-access side channels and at low overhead.
Our insight is that a transaction's size is critically important to the performance and security of the transaction against side channels. A transaction too small leads to leaking fine-grained access patterns and high overhead per-instruction due to the limited degree of cost amortization. A transaction that is too large leads to deterministic abort and execution failure. See \S~\ref{sec:observation} for a preliminary study supporting our observation.
We propose to execute target computations in TSX transactions of proper sizes, that is, fully utilize the CPU cache. Ideally, one can enlarge a transaction to include many instructions as long as including the next instruction does not abort the transaction (e.g., deterministically causing cache misses). To achieve the goal, our approach is to {\it dynamically} insert transaction boundaries instead of doing so statically or manually as in the existing literature. By dynamic program partitioning, various runtime information, including current cache content and utilization, can be taken into account to predict the next cache miss, {\it more accurately}, and to result in larger transactions. The distinction of our research in comparison with existing TSX-based approaches is presented in Table~\ref{tab:distinction}.

We develop a C++ library to materialize dynamic program partitioning inside SGX enclaves. To support generic computations, the library exposes an API and allows developers to encapsulate data types of different access patterns in the target program. Internally, the library partitions a target program and executes the partitioned program in TSX transactions.
Specifically, before entering a TSX transaction, the library prepares the data layout in the main memory to map it to CPU caches with a small footprint.
When running inside the transaction, the library monitors all memory references (through the encapsulated data types), builds a cache model inside the CPU, and analyzes the cache utilization before landing the prediction of which instruction will cause the next cache miss. The prediction result assists the decision-making on when to insert a TSX instruction boundary (e.g., \texttt{xend}) without transaction aborts.
We carefully engineer the system to ensure the cache model has a small footprint in the CPU and does not interfere with the application data.

While our library is generic, we use it to implement a special class of algorithms, namely the external oblivious algorithms, to realize secure data analytics.
Compared with classic ``word''-oblivious algorithms (supported by existing systems such as Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17} and ObliviousML~\cite{DBLP:conf/uss/OhrimenkoSFMNVC16}) and oblivious RAMs~\cite{DBLP:conf/ccs/StefanovDSFRYD13} (supported by ZeroTrace~\cite{DBLP:journals/iacr/SasyGF17} and Prochlo~\cite{DBLP:conf/sosp/BittauEMMRLRKTS17}), external oblivious algorithms have much lower time complexity and is not supported by existing systems to the best of our knowledge.
An external oblivious algorithm accesses data in two places: 1) An external data source, the access to which does not leak secret information, and 2) an internal ``stash'' that needs to be protected from leakage.
We implement an external oblivious algorithm on our library by placing the external data source outside hardware transactions and placing the stash-accessing code inside transactions.
By this means, we implement a variety of data analytics for sorting, shuffle, binary search, $K$-means, etc.
Altogether, the system achieves the notion of cache-miss obliviousness, that is, the trace of cache misses during enclave execution is oblivious to the memory data being accessed. This ensures strong security against most memory-access side-channels, including the physical-level bus tapping.

We evaluate the performance of the built data-analytical system by measuring its execution time.
%Specifically, we compare the transaction size resulted from dynamic partitioning with that from static partitioning (T-SGX) and manual partitioning schemes (Cloak).
We compare the execution time with that of word-oblivious algorithms (used in existing works, Opaque~\cite{DBLP:conf/nsdi/ZhengDBPGS17}). The result shows that our work effectively increases the transaction size and reduces the execution time, both by orders of magnitude.

This work makes the following contributions:

\vspace{2pt}\noindent$\bullet$\textit{
New technique}:
We propose a new technique for partitioning the program dynamically. We build a library to execute the partitioned programs in TSX transactions.
The library works by monitoring cache utilization and asserting a transaction's end upon a full cache.

\vspace{2pt}\noindent$\bullet$\textit{
Secure systems}:
We develop a data-analytical system with strong side-channel security. The system runs external oblivious algorithms on top of the library inside the SGX enclave. It achieves a new security notion, cache-miss obliviousness against all memory-access side channels.

\vspace{2pt}\noindent$\bullet$\textit{
Evaluation}:
We conduct a performance evaluation that shows our system can increase transactions' size and reduce execution time by orders of magnitude compared with the state-of-the-art solutions.



==> text/wheels.tex <==
\section{learning}

\subsection{tables}

{\scriptsize \begin{verbatim} in beamer, see beamer_learn_slides. http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular.2A_environment_-_controlling_table_width
\end{verbatim}}

table with reference~\ref{tab:auth-attack}


\begin{table*}[!htbp] %force in current page, disable float.
\caption{Example of authorized searcher attack}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c|c| }
  \hline
   & $p_0$ & $p_1$ & $p_2$ & $p_3$ & $p_4$ \\ \hline
  $r_a$ & $1$ & $0$ & $1$ & $0$ & $?$ \\ \hline
\end{tabularx}
}
\end{table*}

tabular (not table)

\begin{tabularx}{0.4\textwidth}{ |X|c|c|c| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  label1                    & label2 & label3 & label4 \\ \hline
  \multirow{2}{*}{multi-row} 
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
  \multicolumn{2}{|l|}{multi-column}   & item3''  & item4''  \\  \hline
  \multirow{5}{*}{\begin{sideways}sideways\end{sideways}}
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & \shortstack[l]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & \shortstack[r]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
\end{tabularx}

\subsection{figures}
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\includegraphics[width=0.324\textwidth]{figures2/eff_rand_num_sample0.5.eps}
\caption{Wrapped figure}
\label{fig:perf}
\end{wrapfigure}

\ifdefined\TTUT
\begin{figure}[!ht]
\begin{center}
    \includegraphics[angle=90, width=0.45\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
\end{center}
%\vspace{-0.15in}
\caption{Easy figure}\label{fig:easy}
\vspace{-0.10in}\end{figure}

\begin{figure*}[!ht]
  \begin{center}
  %\goodgap
    \subfloat[Rotated]{%
      \includegraphics[angle=90, width=0.3\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
      \label{exp:rand_num_1}%
    }%
    %\hspace{-0.2cm}%
    \subfloat[With more shared threads]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_num_sample2.eps}%
      \label{exp:rand_num_2}%
    }%
    \subfloat[With sample ratio]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_sample_num10.eps}%
      \label{exp:rand_sample}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Performance of optimization algorithm with random graph}\label{fig:complex}\vspace{-0.10in}
\end{figure*}
\fi

\subsection{algorithms}
\begin{algorithm}[h]
\caption{range-query(range $R$)}\small \label{alg:rangequery}
\begin{algorithmic}[1]
  \boldnext\State $\omega_R\leftarrow $ lowest-common-ancestor($R$) \Comment{comments: line number boldened}
  \State $\lambda\leftarrow $ DHT-lookup($f_{md}(\omega_R)$)
  \ForAll{$p \in P$} \Comment{comments: loop over all items}
    \State manipulate each term $p$
  \EndFor
  \If{$\lambda == NULL \And 1 \leq 0$}
      \State \Return lookup($R$.top\_left\_corner)
  \ElsIf{$R\subseteq{\lambda}$}
      \State \Return the keys of $\lambda$ that are in the range $R$
  \Else
      \State \Return recursive-forward($R$, $\omega_R$)
  \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{equations}
\begin{eqnarray}
u &=& \sum_{l=0}^{n-1}{u_l} \mod{q} %\nonumber \\
=(\sum_{l=0}^{n-1}{ \sum_{j=0}^{c-1}{u_{l-j, j}} \mod{q}})\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{ \sum_{l=0}^{n-1}{ u_{l-j, j} } })\mod{q} %\nonumber \\
=(\sum_{j=0}^{c-1}{ \sum_{i=-j}^{n-1-j}{ u_{i, j} } })\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{\sum_{i=0}^{n-1}{ u_{i, j} } }) mod q
= (\sum_{i=0}^{n-1}{ \sum_{j=0}^{c-1}{ u_{i, j} }\mod{q} })\mod{q} \nonumber \\
&=& \sum_{i=0}^{n-1}{ v_i }\mod{q} = \sum_{i=0}^{n-1}{ v_i } = v
\end{eqnarray}

With right brace
\begin{eqnarray}
\underline{\sigma}, \epsilon \rightarrow{}\underline{\beta_*}
\begin{cases}
\begin{rcases}
\begin{rcases}
& \sum_{\forall\beta_*>1}{(\beta_* - 1)} \\
& \sum_{\forall\beta_*<1}{(1 - \beta_*)} \\  
\end{rcases} \rightarrow{} \underline{X_1}\% \\
\sum_{\beta_*<1}{1} \rightarrow{} \underline{X_2}\%
\end{rcases}
\end{cases}
 \rightarrow{\beta}
\end{eqnarray}

\subsection{listing}
\lstset{language=SQL, style=Oracle, caption={Rewritten query against a single view table},label=sql:rewritten}
\lstset{frame=lrbt,xleftmargin=\fboxsep,xrightmargin=-\fboxsep} %with bounding box at l(eft)r(right)b(ottom)t(op)
%or you can replace it with "frame=single"
\begin{lstlisting}
  SELECT A, C FROM viewtable
  ORDER BY C LIMIT arg.k
\end{lstlisting}

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
public void OnTouchEvent(MotionEvent e) {
Bitmap LoadPicture(String path) {
    ...
    *Bitmap bm = BitmapFactory.decodeFile(file)*;
    return bm;
}

void EditPicture(Bitmap bm) {
    //heavy computational picture editing
    int i = 10 (* $*$ *); //escape to plot * literatelly instead of bolden text
    bm.getPixels(pix, 0, mPhotoWidth, 0, 0, mPhotoWidth, mPhotoHeight);
    for(every pixel) {
      ...
    }  
    
    //embed location information into picture
    (* $*$*)Location loc = getLastKnownLocation(Provider)*;
    (* $*$*)double longitude = loc.getLongitude()*;
    (* $*$*)double latitude = loc.getLatitude()*;
    (* $*$*)EmbedLocation(bm, longitude, latitude);*
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Privacy-preserving Offloading Example}
\label{figure:MotivatingExample}
\end{figure}


\subsection{fbox}
\begin{center}
\fbox{This is a sample statement}
\end{center}

\begin{center}
\fbox{\parbox{0.90\linewidth}{
This is a long long long statement: 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
}}
\end{center}



\subsection{misc}
\begin{itemize}
  \item cmark $\cmark$ and xmark $\xmark$
  \item bold math type $\boldsymbol{<v_0, k>}$
  \item use other than default font size: {``\fontsize{8.5}{9} this's in font size 8.5''}. (second param. should be 1.2$\times$ first param. which is font size
  \item show tilde in url, use \textasciitilde{} rather than \~{}
  \item strike out text, \sout{text/$12$ removed}
  \item color, {\color{red}red}{\color{green}green}
  \item[$\bullet$] big bullet on each item
  \item circled text \circled{2}
  \item A white number inside a black circle: \ballnumber{37}
  \item empty set (beautiful version) $\varnothing$ (needs ``\\usepackage\{amssymb\}''), which renames emptyset, $\emptyset$
  \item stackrel $\stackrel[c]{a}{=}$
\end{itemize}

citation for long breakable url~\cite{me:mssgx}

